Generative Retrieval Meets Multi-Graded Relevance

Generative retrieval represents a novel approach to information retrieval. It uses an encoder-decoder architecture to directly produce relevant document identifiers (docids) for queries. While this method offers benefits, current approaches are limited to scenarios with binary relevance data, overlooking the potential for documents to have multi-graded relevance. Extending generative retrieval to accommodate multi-graded relevance poses challenges, including the need to reconcile likelihood probabilities for docid pairs and the possibility of multiple relevant documents sharing the same identifier. To address these challenges, we introduce a framework called GRaded Generative Retrieval (GR$^2$). GR$^2$ focuses on two key components: ensuring relevant and distinct identifiers, and implementing multi-graded constrained contrastive training. First, we create identifiers that are both semantically relevant and sufficiently distinct to represent individual documents effectively. This is achieved by jointly optimizing the relevance and distinctness of docids through a combination of docid generation and autoencoder models. Second, we incorporate information about the relationship between relevance grades to guide the training process. We use a constrained contrastive training strategy to bring the representations of queries and the identifiers of their relevant documents closer together, based on their respective relevance grades. Extensive experiments on datasets with both multi-graded and binary relevance demonstrate the effectiveness of GR$^2$.

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Abstract and Section \ref{sec:introduction}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:conclusion}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:introduction}, Section \ref{formulation} and Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}, Appendix \ref{appendix-datasets}, and Appendix \ref{appendix-implementation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:\answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:conclusion}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix \ref{appendix-implementation}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section \ref{sec:experiments}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We didn't introduce new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We didn't conduct crowdsourcing experiments and research with human subjects. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work only focuses on generative retrieval with multi-graded relevance. And it has no potential risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}



==> sections/ref.tex <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
 @String{AMSTrans = "American Mathematical Society Translations" }
 @String{AMSTrans = "Amer. Math. Soc. Transl." }
 @String{BullAMS = "Bulletin of the American Mathematical Society" }
 @String{BullAMS = "Bull. Amer. Math. Soc." }
 @String{ProcAMS = "Proceedings of the American Mathematical Society" }
 @String{ProcAMS = "Proc. Amer. Math. Soc." }
 @String{TransAMS = "Transactions of the American Mathematical Society" }
 @String{TransAMS = "Trans. Amer. Math. Soc." }

 %ACM
 @String{CACM = "Communications of the {ACM}" }
 @String{CACM = "Commun. {ACM}" }
 @String{CompServ = "Comput. Surveys" }
 @String{JACM = "J. ACM" }
 @String{ACMMathSoft = "{ACM} Transactions on Mathematical Software" }
 @String{ACMMathSoft = "{ACM} Trans. Math. Software" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newsletter" }
 @String{SIGNUM = "{ACM} {SIGNUM} Newslett." }

 @String{AmerSocio = "American Journal of Sociology" }
 @String{AmerStatAssoc = "Journal of the American Statistical Association" }
 @String{AmerStatAssoc = "J. Amer. Statist. Assoc." }
 @String{ApplMathComp = "Applied Mathematics and Computation" }
 @String{ApplMathComp = "Appl. Math. Comput." }
 @String{AmerMathMonthly = "American Mathematical Monthly" }
 @String{AmerMathMonthly = "Amer. Math. Monthly" }
 @String{BIT = "{BIT}" }
 @String{BritStatPsych = "British Journal of Mathematical and Statistical
          Psychology" }
 @String{BritStatPsych = "Brit. J. Math. Statist. Psych." }
 @String{CanMathBull = "Canadian Mathematical Bulletin" }
 @String{CanMathBull = "Canad. Math. Bull." }
 @String{CompApplMath = "Journal of Computational and Applied Mathematics" }
 @String{CompApplMath = "J. Comput. Appl. Math." }
 @String{CompPhys = "Journal of Computational Physics" }
 @String{CompPhys = "J. Comput. Phys." }
 @String{CompStruct = "Computers and Structures" }
 @String{CompStruct = "Comput. \& Structures" }
 @String{CompJour = "The Computer Journal" }
 @String{CompJour = "Comput. J." }
 @String{CompSysSci = "Journal of Computer and System Sciences" }
 @String{CompSysSci = "J. Comput. System Sci." }
 @String{Computing = "Computing" }
 @String{ContempMath = "Contemporary Mathematics" }
 @String{ContempMath = "Contemp. Math." }
 @String{Crelle = "Crelle's Journal" }
 @String{GiornaleMath = "Giornale di Mathematiche" }
 @String{GiornaleMath = "Giorn. Mat." } % didn't find in AMS MR., ibid.

 %IEEE
 @String{Computer = "{IEEE} Computer" }
 @String{IEEETransComp = "{IEEE} Transactions on Computers" }
 @String{IEEETransComp = "{IEEE} Trans. Comput." }
 @String{IEEETransAC = "{IEEE} Transactions on Automatic Control" }
 @String{IEEETransAC = "{IEEE} Trans. Automat. Control" }
 @String{IEEESpec = "{IEEE} Spectrum" } % didn't find in AMS MR
 @String{ProcIEEE = "Proceedings of the {IEEE}" }
 @String{ProcIEEE = "Proc. {IEEE}" } % didn't find in AMS MR
 @String{IEEETransAeroElec = "{IEEE} Transactions on Aerospace and Electronic
     Systems" }
 @String{IEEETransAeroElec = "{IEEE} Trans. Aerospace Electron. Systems" }

 @String{IMANumerAna = "{IMA} Journal of Numerical Analysis" }
 @String{IMANumerAna = "{IMA} J. Numer. Anal." }
 @String{InfProcLet = "Information Processing Letters" }
 @String{InfProcLet = "Inform. Process. Lett." }
 @String{InstMathApp = "Journal of the Institute of Mathematics and
     its Applications" }
 @String{InstMathApp = "J. Inst. Math. Appl." }
 @String{IntControl = "International Journal of Control" }
 @String{IntControl = "Internat. J. Control" }
 @String{IntNumerEng = "International Journal for Numerical Methods in
     Engineering" }
 @String{IntNumerEng = "Internat. J. Numer. Methods Engrg." }
 @String{IntSuper = "International Journal of Supercomputing Applications" }
 @String{IntSuper = "Internat. J. Supercomputing Applic." } % didn't find
%% in AMS MR
 @String{Kibernetika = "Kibernetika" }
 @String{JResNatBurStand = "Journal of Research of the National Bureau
     of Standards" }
 @String{JResNatBurStand = "J. Res. Nat. Bur. Standards" }
 @String{LinAlgApp = "Linear Algebra and its Applications" }
 @String{LinAlgApp = "Linear Algebra Appl." }
 @String{MathAnaAppl = "Journal of Mathematical Analysis and Applications" }
 @String{MathAnaAppl = "J. Math. Anal. Appl." }
 @String{MathAnnalen = "Mathematische Annalen" }
 @String{MathAnnalen = "Math. Ann." }
 @String{MathPhys = "Journal of Mathematical Physics" }
 @String{MathPhys = "J. Math. Phys." }
 @String{MathComp = "Mathematics of Computation" }
 @String{MathComp = "Math. Comp." }
 @String{MathScand = "Mathematica Scandinavica" }
 @String{MathScand = "Math. Scand." }
 @String{TablesAidsComp = "Mathematical Tables and Other Aids to Computation" }
 @String{TablesAidsComp = "Math. Tables Aids Comput." }
 @String{NumerMath = "Numerische Mathematik" }
 @String{NumerMath = "Numer. Math." }
 @String{PacificMath = "Pacific Journal of Mathematics" }
 @String{PacificMath = "Pacific J. Math." }
 @String{ParDistComp = "Journal of Parallel and Distributed Computing" }
 @String{ParDistComp = "J. Parallel and Distrib. Comput." } % didn't find
%% in AMS MR
 @String{ParComputing = "Parallel Computing" }
 @String{ParComputing = "Parallel Comput." }
 @String{PhilMag = "Philosophical Magazine" }
 @String{PhilMag = "Philos. Mag." }
 @String{ProcNAS = "Proceedings of the National Academy of Sciences
                    of the USA" }
 @String{ProcNAS = "Proc. Nat. Acad. Sci. U. S. A." }
 @String{Psychometrika = "Psychometrika" }
 @String{QuartMath = "Quarterly Journal of Mathematics, Oxford, Series (2)" }
 @String{QuartMath = "Quart. J. Math. Oxford Ser. (2)" }
 @String{QuartApplMath = "Quarterly of Applied Mathematics" }
 @String{QuartApplMath = "Quart. Appl. Math." }
 @String{RevueInstStat = "Review of the International Statisical Institute" }
 @String{RevueInstStat = "Rev. Inst. Internat. Statist." }

 %SIAM
 @String{JSIAM = "Journal of the Society for Industrial and Applied
     Mathematics" }
 @String{JSIAM = "J. Soc. Indust. Appl. Math." }
 @String{JSIAMB = "Journal of the Society for Industrial and Applied
     Mathematics, Series B, Numerical Analysis" }
 @String{JSIAMB = "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." }
 @String{SIAMAlgMeth = "{SIAM} Journal on Algebraic and Discrete Methods" }
 @String{SIAMAlgMeth = "{SIAM} J. Algebraic Discrete Methods" }
 @String{SIAMAppMath = "{SIAM} Journal on Applied Mathematics" }
 @String{SIAMAppMath = "{SIAM} J. Appl. Math." }
 @String{SIAMComp = "{SIAM} Journal on Computing" }
 @String{SIAMComp = "{SIAM} J. Comput." }
 @String{SIAMMatrix = "{SIAM} Journal on Matrix Analysis and Applications" }
 @String{SIAMMatrix = "{SIAM} J. Matrix Anal. Appl." }
 @String{SIAMNumAnal = "{SIAM} Journal on Numerical Analysis" }
 @String{SIAMNumAnal = "{SIAM} J. Numer. Anal." }
 @String{SIAMReview = "{SIAM} Review" }
 @String{SIAMReview = "{SIAM} Rev." }
 @String{SIAMSciStat = "{SIAM} Journal on Scientific and Statistical
     Computing" }
 @String{SIAMSciStat = "{SIAM} J. Sci. Statist. Comput." }

 @String{SoftPracExp = "Software Practice and Experience" }
 @String{SoftPracExp = "Software Prac. Experience" } % didn't find in AMS MR
 @String{StatScience = "Statistical Science" }
 @String{StatScience = "Statist. Sci." }
 @String{Techno = "Technometrics" }
 @String{USSRCompMathPhys = "{USSR} Computational Mathematics and Mathematical
     Physics" }
 @String{USSRCompMathPhys = "{U. S. S. R.} Comput. Math. and Math. Phys." }
 @String{VLSICompSys = "Journal of {VLSI} and Computer Systems" }
 @String{VLSICompSys = "J. {VLSI} Comput. Syst." }
 @String{ZAngewMathMech = "Zeitschrift fur Angewandte Mathematik und
     Mechanik" }
 @String{ZAngewMathMech = "Z. Angew. Math. Mech." }
 @String{ZAngewMathPhys = "Zeitschrift fur Angewandte Mathematik und Physik" }
 @String{ZAngewMathPhys = "Z. Angew. Math. Phys." }

% Publishers % ================================================= |

 @String{Academic = "Academic Press" }
 @String{ACMPress = "{ACM} Press" }
 @String{AdamHilger = "Adam Hilger" }
 @String{AddisonWesley = "Addison-Wesley" }
 @String{AllynBacon = "Allyn and Bacon" }
 @String{AMS = "American Mathematical Society" }
 @String{Birkhauser = "Birkha{\"u}ser" }
 @String{CambridgePress = "Cambridge University Press" }
 @String{Chelsea = "Chelsea" }
 @String{ClaredonPress = "Claredon Press" }
 @String{DoverPub = "Dover Publications" }
 @String{Eyolles = "Eyolles" }
 @String{HoltRinehartWinston = "Holt, Rinehart and Winston" }
 @String{Interscience = "Interscience" }
 @String{JohnsHopkinsPress = "The Johns Hopkins University Press" }
 @String{JohnWileySons = "John Wiley and Sons" }
 @String{Macmillan = "Macmillan" }
 @String{MathWorks = "The Math Works Inc." }
 @String{McGrawHill = "McGraw-Hill" }
 @String{NatBurStd = "National Bureau of Standards" }
 @String{NorthHolland = "North-Holland" }
 @String{OxfordPress = "Oxford University Press" }  %address Oxford or London?
 @String{PergamonPress = "Pergamon Press" }
 @String{PlenumPress = "Plenum Press" }
 @String{PrenticeHall = "Prentice-Hall" }
 @String{SIAMPub = "{SIAM} Publications" }
 @String{Springer = "Springer-Verlag" }
 @String{TexasPress = "University of Texas Press" }
 @String{VanNostrand = "Van Nostrand" }
 @String{WHFreeman = "W. H. Freeman and Co." }

%Entries

@Article{Abril07,
  author        = "Patricia S. Abril and Robert Plant",
  title         = "The patent holder's dilemma: Buy, sell, or troll?",
  journal       = "Communications of the ACM",
  volume        = "50",
  number        = "1",
  month         = jan,
  year          = "2007",
  pages         = "36--44",
  doi           = "10.1145/1188913.1188915",
  url           = "http://doi.acm.org/10.1145/1219092.1219093",
  note          = "",
}

@Article{Cohen07,
  author        = "Sarah Cohen and Werner Nutt and Yehoshua Sagic",
  title         = "Deciding equivalances among conjunctive aggregate queries",
  journal       = JACM,
  articleno     = 5,
  numpages      = 50,
  volume        = 54,
  number        = 2,
  month         = apr,
  year          = 2007,
  doi           = "10.1145/1219092.1219093",
  url           = "http://doi.acm.org/10.1145/1219092.1219093",
  acmid         = 1219093,
}


@periodical{JCohen96,
  key =          "Cohen",
  editor =       "Jacques Cohen",
  title =        "Special issue: Digital Libraries",
  journal =      CACM,
  volume =       "39",
  number =       "11",
  month =        nov,
  year =         "1996",
}


@Book{Kosiur01,
  author =       "David Kosiur",
  title =        "Understanding Policy-Based Networking",
  publisher =    "Wiley",
  year =         "2001",
  address =      "New York, NY",
  edition =      "2nd.",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  month =        "",
  note =         "",
}




@Book{Harel79,
  author =       "David Harel",
  year =         "1979",
  title =        "First-Order Dynamic Logic",
  series =       "Lecture Notes in Computer Science",
  volume =       "68",
  address =      "New York, NY",
  publisher =    "Springer-Verlag",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09237-4",
  editor =       "",
  number =       "",
  month =        "",
  note =         "",
}


@Inbook{Editor00,
  author =       "",
  editor =       "Ian Editor",
  title =        "The title of book one",
  subtitle =     "The book subtitle",
  series =       "The name of the series one",
  year =         "2007",
  volume =       "9",
  address =      "Chicago",
  edition =      "1st.",
  publisher =    "University of Chicago Press",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09456-9",
  chapter =      "",
  pages =        "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}

%
@InBook{Editor00a,
  author =       "",
  editor =       "Ian Editor",
  title =        "The title of book two",
  subtitle =     "The book subtitle",
  series =       "The name of the series two",
  year =         "2008",
  address =      "Chicago",
  edition =      "2nd.",
  publisher =    "University of Chicago Press",
  doi =          "10.1007/3-540-09237-4",
  url =          "http://dx.doi.org/10.1007/3-540-09456-9",
  volume =       "",
  chapter =      "100",
  pages =        "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}


% incollection (has an editor, title, and possibly a booktitle)
@Incollection{Spector90,
  author =       "Asad Z. Spector",
  title =        "Achieving application requirements",
  booktitle =    "Distributed Systems",
  publisher =    "ACM Press",
  address =      "New York, NY",
  year =         "1990",
  edition =      "2nd.",
  chapter =      "",
  editor =       "Sape Mullender",
  pages =        "19--33",
  doi =          "10.1145/90417.90738",
  url =          "http://doi.acm.org/10.1145/90417.90738",
  volume =       "",
  number =       "",
  series =       "",
  type =         "",
  month =        "",
  note =         "",
}


% incollection (has an editor, title, and possibly a booktitle)
@Incollection{Douglass98,
  author =       "Bruce P. Douglass and David Harel and Mark B. Trakhtenbrot",
  title =        "Statecarts in use: structured analysis and object-orientation",
  series =       "Lecture Notes in Computer Science",
  booktitle =    "Lectures on Embedded Systems",
  publisher =    "Springer-Verlag",
  address =      "London",
  volume =       "1494",
  year =         "1998",
  chapter =      "",
  editor =       "Grzegorz Rozenberg and Frits W. Vaandrager",
  pages =        "368--394",
  doi =          "10.1007/3-540-65193-4_29",
  url =          "http://dx.doi.org/10.1007/3-540-65193-4_29",
  edition =      "",
  number =       "",
  type =         "",
  month =        "",
  note =         "",
}


@Book{Knuth97,
  author =       "Donald E. Knuth",
  title =        "The Art of Computer Programming, Vol. 1: Fundamental Algorithms (3rd. ed.)",
  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
  year =         "1997",
  address =      "",
  edition =      "",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  month =        "",
  note =         "",
}


@Book{Knuth98,
  author =       "Donald E. Knuth",
  year =         "1998",
  title =        "The Art of Computer Programming",
  series =       "Fundamental Algorithms",
  volume =       "1",
  edition =      "3rd",
  address =      "",
  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
  doi =          "",
  url =          "",
  editor =       "",
  number =       "",
  month =        "",
  note =         "(book)",
}

%Inbook{Knuth97,
%  author =       "Donald E. Knuth",
%  title =        "The Art of Computer Programming",
%  booktitle =    "the booktitle",
%  edition =      "3",
%  volume =       "1",
%  year =         "1997",
%  publisher =    "Addison Wesley Longman Publishing Co., Inc.",
%  editor =       "",
%  number =       "",
%  series =       "Fundamental Algorithms",
%  type =         "",
%  chapter =      "",
%  pages =        "",
%  address =      "",
%  month =        "",
%  note =         "(inbook)",
%}

%INBOOK{DK:73-inbook-full,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (inbook w series)",
%   volume = 1,
%   series = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   edition = "Second",
%   month = "10~" # jan,
%   year = "1973",
%   type = "Section",
%   chapter = "1.2",
%   pages = "10--119",
%   note = "Full INBOOK entry (w series)",
%}

%INcollection{DK:74-incoll,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (incoll)",
%   volume = 1,
%   booktitle = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   month = "10~" # jan,
%   year = "1974",
%   pages = "10--119",
%   editor = "Bernard Rous",
%   note = "This is a full incoll entry with an editor",
%}

%INcollection{DK:75-incollws,
%   author = "Donald E. Knuth",
%   title = "Fundamental Algorithms (incoll w series)",
%   volume = 1,
%   booktitle = "The Art of Computer Programming",
%   series = "The Art of Computer Programming",
%   publisher = "Addison-Wesley",
%   address = "Reading, Massachusetts",
%   month = "10~" # jan,
%   year = "1975",
%   pages = "10--119",
%   editor = "Bernard Rous",
%   note = "This is a full incoll entry with an editor and series",
%}


@incollection{GM05,
Author= "Dan Geiger and Christopher Meek",
Title= "Structured Variational Inference Procedures and their Realizations (as incol)",
Year= 2005,
Booktitle="Proceedings of Tenth International Workshop on Artificial Intelligence and Statistics, {\rm The Barbados}",
Publisher="The Society for Artificial Intelligence and Statistics",
Month= jan,
Editors= "Z. Ghahramani and R. Cowell"
}

@Inproceedings{Smith10,
  author =       "Stan W. Smith",
  title =        "An experiment in bibliographic mark-up: Parsing metadata for XML export",
  booktitle =    "Proceedings of the 3rd. annual workshop on Librarians and Computers",
  series =       "LAC '10",
  editor =       "Reginald N. Smythe and Alexander Noble",
  volume =       "3",
  year =         "2010",
  publisher =    "Paparazzi Press",
  address =      "Milan Italy",
  pages =        "422--431",
  doi =          "99.9999/woot07-S422",
  url =          "http://dx.doi.org/99.0000/woot07-S422",
  number =       "",
  month =        "",
  organization = "",
  note =         "",
}

@Inproceedings{VanGundy07,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2007,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '07",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  articleno =    {Paper 7},
  numpages =     9,
}

@Inproceedings{VanGundy08,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2008,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '08",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  articleno =    7,
  numpages =     2,
  pages =        "99-100",
}

@Inproceedings{VanGundy09,
  author =       "Matthew Van Gundy and Davide Balzarotti and Giovanni Vigna",
  year =         2009,
  title =        "Catch me, if you can: Evading network signatures with web-based polymorphic worms",
  booktitle =    "Proceedings of the first USENIX workshop on Offensive Technologies",
  series =       "WOOT '09",
  publisher =    "USENIX Association",
  address =      "Berkley, CA",
  pages =        "90--100",
}

@Inproceedings{Andler79,
  author =       "Sten Andler",
  title =        "Predicate Path expressions",
  booktitle =    "Proceedings of the 6th. ACM SIGACT-SIGPLAN symposium on Principles of Programming Languages",
  series =       "POPL '79",
  year =         "1979",
  publisher =    "ACM Press",
  address =      "New York, NY",
  pages =        "226--236",
  doi =          "10.1145/567752.567774",
  url =          "http://doi.acm.org/10.1145/567752.567774",
  editor =       "",
  volume =       "",
  number =       "",
  month =        "",
  organization = "",
  note =         "",
}

@Techreport{Harel78,
  author =       "David Harel",
  year =         "1978",
  title =        "LOGICS of Programs: AXIOMATICS and DESCRIPTIVE POWER",
  institution =  "Massachusetts Institute of Technology",
  type =         "MIT Research Lab Technical Report",
  number =       "TR-200",
  address =      "Cambridge, MA",
  month =        "",
  note =         "",
}

@MASTERSTHESIS{anisi03,
author = {David A. Anisi},
title = {Optimal Motion Control of a Ground Vehicle},
school = {Royal Institute of Technology (KTH), Stockholm, Sweden},
intitution = {FOI-R-0961-SE, Swedish Defence Research Agency (FOI)},
year = {2003},
}


@Phdthesis{Clarkson85,
  author =       "Kenneth L. Clarkson",
  year =         "1985",
  title =        "Algorithms for Closest-Point Problems (Computational Geometry)",
  school =       "Stanford University",
  address =      "Palo Alto, CA",
  note =         "UMI Order Number: AAT 8506171",
  type =         "",
  month =        "",
}


@online{Thornburg01,
  author =       "Harry Thornburg",
  year =         "2001",
  title =        "Introduction to Bayesian Statistics",
  url =          "http://ccrma.stanford.edu/~jos/bayes/bayes.html",
  month =        mar,
  lastaccessed = "March 2, 2005",
}


@online{Ablamowicz07,
  author =       "Rafal Ablamowicz and Bertfried Fauser",
  year =         "2007",
  title =        "CLIFFORD: a Maple 11 Package for Clifford Algebra Computations, version 11",
  url =          "http://math.tntech.edu/rafal/cliff11/index.html",
  lastaccessed = "February 28, 2008",
}


@misc{Poker06,
  author =       "Poker-Edge.Com",
  year =         "2006",
  month =        mar,
  title =        "Stats and Analysis",
  lastaccessed = "June 7, 2006",
  url =          "http://www.poker-edge.com/stats.php",
}

@misc{Obama08,
  author        = "Barack Obama",
  year          = "2008",
  title         = "A more perfect union",
  howpublished  = "Video",
  day           = "5",
  url           = "http://video.google.com/videoplay?docid=6528042696351994555",
  month         = mar,
  lastaccessed  = "March 21, 2008",
  note          =  "",
}

@misc{JoeScientist001,
  author =       "Joseph Scientist",
  year =         "2009",
  title =        "The fountain of youth",
  note =         "Patent No. 12345, Filed July 1st., 2008, Issued Aug. 9th., 2009",
  url =          "",
  howpublished = "",
  month =        aug,
  lastaccessed = "",
}


@Inproceedings{Novak03,
  author =       "Dave Novak",
  title =        "Solder man",
  booktitle =    "ACM SIGGRAPH 2003 Video Review on Animation theater Program: Part I - Vol. 145 (July 27--27, 2003)",
  year =         "2003",
  publisher =    "ACM Press",
  address =      "New York, NY",
  pages =        "4",
  month =        "March 21, 2008",
  doi =          "99.9999/woot07-S422",
  url =          "http://video.google.com/videoplay?docid=6528042696351994555",
  note =         "",
  howpublished = "Video",
  editor =       "",
  volume =       "",
  number =       "",
  series =       "",
  organization = "",
  distinctURL = 1
}


@article{Lee05,
  author =       "Newton Lee",
  year =         "2005",
  title =        "Interview with Bill Kinder: January 13, 2005",
  journal =      "Comput. Entertain.",
  eid =          "4",
  volume =       "3",
  number =       "1",
  month =        "Jan.-March",
  doi =          "10.1145/1057270.1057278",
  url =          "http://doi.acm.org/10.1145/1057270.1057278",
  howpublished = "Video",
  note =         "",
}

@article{rous08,
  author =       "Bernard Rous",
  year =         "2008",
  title =        "The Enabling of Digital Libraries",
  journal =      "Digital Libraries",
  volume =       "12",
  number =       "3",
  month =        jul,
  articleno =    "Article~5",
  doi =          "",
  url =          "",
  howpublished = "",
  note =         "To appear",
}

@article{384253,
 author = {Werneck,, Renato and Setubal,, Jo\~{a}o and da Conceic\~{a}o,, Arlindo},
 title = {(old) Finding minimum congestion spanning trees},
 journal = {J. Exp. Algorithmics},
 volume = {5},
 year = {2000},
 issn = {1084-6654},
 pages = {11},
 doi = {http://doi.acm.org/10.1145/351827.384253},
 publisher = {ACM},
 address = {New York, NY, USA},
 }


@article{Werneck:2000:FMC:351827.384253,
 author = {Werneck, Renato and Setubal, Jo\~{a}o and da Conceic\~{a}o, Arlindo},
 title = {(new) Finding minimum congestion spanning trees},
 journal = {J. Exp. Algorithmics},
 volume = 5,
 month = dec,
 year = 2000,
 issn = {1084-6654},
 articleno = 11,
 url = {http://portal.acm.org/citation.cfm?id=351827.384253},
 doi = {10.1145/351827.384253},
 acmid = 384253,
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{1555162,
 author = {Conti, Mauro and Di Pietro, Roberto and Mancini, Luigi V. and Mei, Alessandro},
 title = {(old) Distributed data source verification in wireless sensor networks},
 journal = {Inf. Fusion},
 volume = {10},
 number = {4},
 year = {2009},
 issn = {1566-2535},
 pages = {342--353},
 doi = {http://dx.doi.org/10.1016/j.inffus.2009.01.002},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 }

@article{Conti:2009:DDS:1555009.1555162,
 author = {Conti, Mauro and Di Pietro, Roberto and Mancini, Luigi V. and Mei, Alessandro},
 title = {(new) Distributed data source verification in wireless sensor networks},
 journal = {Inf. Fusion},
 volume = {10},
 number = {4},
 month = oct,
 year = {2009},
 issn = {1566-2535},
 pages = {342--353},
 numpages = {12},
 url = {http://portal.acm.org/citation.cfm?id=1555009.1555162},
 doi = {10.1016/j.inffus.2009.01.002},
 acmid = {1555162},
 publisher = {Elsevier Science Publishers B. V.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Clone detection, Distributed protocol, Securing data fusion, Wireless sensor networks},
}

@inproceedings{Li:2008:PUC:1358628.1358946,
 author = {Li, Cheng-Lun and Buyuktur, Ayse G. and Hutchful, David K. and Sant, Natasha B. and Nainwal, Satyendra K.},
 title = {Portalis: using competitive online interactions to support aid initiatives for the homeless},
 booktitle = {CHI '08 extended abstracts on Human factors in computing systems},
 year = {2008},
 isbn = {978-1-60558-012-X},
 location = {Florence, Italy},
 pages = {3873--3878},
 numpages = {6},
 url = {http://portal.acm.org/citation.cfm?id=1358628.1358946},
 doi = {10.1145/1358628.1358946},
 acmid = {1358946},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {cscw, distributed knowledge acquisition, incentive design, online games, recommender systems, reputation systems, user studies, virtual community},
}

@book{Hollis:1999:VBD:519964,
 author = {Hollis, Billy S.},
 title = {Visual Basic 6: Design, Specification, and Objects with Other},
 year = {1999},
 isbn = {0130850845},
 edition = {1st},
 publisher = {Prentice Hall PTR},
 address = {Upper Saddle River, NJ, USA},
 }


@book{Goossens:1999:LWC:553897,
 author = {Goossens, Michel and Rahtz, S. P. and Moore, Ross and Sutor, Robert S.},
 title = {The  Latex Web Companion: Integrating TEX, HTML, and XML},
 year = {1999},
 isbn = {0201433117},
 edition = {1st},
 publisher = {Addison-Wesley Longman Publishing Co., Inc.},
 address = {Boston, MA, USA},
 }

% need to test genres for errant isbn output

% techreport
@techreport{897367,
 author = {Buss, Jonathan F. and Rosenberg, Arnold L. and Knott, Judson D.},
 title = {Vertex Types in Book-Embeddings},
 year = {1987},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Aumass_cs%3Ancstrl.umassa_cs%2F%2FUM-CS-1987-018},
 publisher = {University of Massachusetts},
 address = {Amherst, MA, USA},
 }
@inproceedings{chen2022gere,
  title={GERE: Generative Evidence Retrieval for Fact Verification},
  author={Chen, Jiangui and Zhang, Ruqing and Guo, Jiafeng and Fan, Yixing and Cheng, Xueqi},
  booktitle={Proceedings of the 45th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={2184--2189},
  year={2022}
}
@inproceedings{petroni2021kilt,
  title={KILT: a Benchmark for Knowledge Intensive Language Tasks},
  author={Petroni, Fabio and Piktus, Aleksandra and Fan, Angela and Lewis, Patrick and Yazdani, Majid and De Cao, Nicola and Thorne, James and Jernite, Yacine and Karpukhin, Vladimir and Maillard, Jean and others},
  booktitle={Proceedings of the 2021 Conf.\ of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={2523--2544},
  year={2021}
}
@techreport{Buss:1987:VTB:897367,
 author = {Buss, Jonathan F. and Rosenberg, Arnold L. and Knott, Judson D.},
 title = {Vertex Types in Book-Embeddings},
 year = {1987},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Aumass_cs%3Ancstrl.umassa_cs%2F%2FUM-CS-1987-018},
 publisher = {University of Massachusetts},
 address = {Amherst, MA, USA},
 }

% whole proceedings

@proceedings{Czerwinski:2008:1358628,
 author = {},
 note = {General Chair-Czerwinski, Mary and General Chair-Lund, Arnie and Program Chair-Tan, Desney},
 title = {CHI '08: CHI '08 extended abstracts on Human factors in computing systems},
 year = {2008},
 isbn = {978-1-60558-012-X},
 location = {Florence, Italy},
 order_no = {608085},
 publisher = {ACM},
 address = {New York, NY, USA},
 }

% phdthesis

@phdthesis{Clarkson:1985:ACP:911891,
 author = {Clarkson, Kenneth Lee},
 advisor = {Yao, Andrew C.},
 title = {Algorithms for Closest-Point Problems (Computational Geometry)},
 year = {1985},
 note = {AAT 8506171},
 school = {Stanford University},
 address = {Stanford, CA, USA},
 }
% school is being picked up -- but not publisher (which is OK)
% Also -- the title is NOT being output in italics !!! Arrrrgh! - I fixed it. :-)


%%% compare with 'old'
%%% atsign-Phdthesis{Clarkson85,
%%%  author =       "Kenneth L. Clarkson",
%%%  year =         "1985",
%%%  title =        "Algorithms for Closest-Point Problems (Computational Geometry)",
%%%  school =       "Stanford University",
%%%  address =      "Palo Alto, CA",
%%%  note =         "UMI Order Number: AAT 8506171",
%%%  type =         "",
%%%  month =        "",
%%%}

% A bibliography
@Article{1984:1040142,
 key = {{$\!\!$}},
 journal = {SIGCOMM Comput. Commun. Rev.},
 year = {1984},
 issn = {0146-4833},
 volume = {13-14},
 number = {5-1},
 issue_date = {January/April 1984},
 publisher = {ACM},
 address = {New York, NY, USA},
 }


% grinder
@inproceedings{2004:ITE:1009386.1010128,
 key = {IEEE},
 title = {IEEE TCSC Executive Committee},
 booktitle = {Proceedings of the IEEE International Conference on Web Services},
 series = {ICWS '04},
 year = {2004},
 isbn = {0-7695-2167-3},
 pages = {21--22},
 url = {http://dx.doi.org/10.1109/ICWS.2004.64},
 doi = {http://dx.doi.org/10.1109/ICWS.2004.64},
 acmid = {1010128},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}

% div book
@book{Mullender:1993:DS:302430,
 editor = {Mullender, Sape},
 title = {Distributed systems (2nd Ed.)},
 year = {1993},
 isbn = {0-201-62427-3},
 publisher = {ACM Press/Addison-Wesley Publishing Co.},
 address = {New York, NY, USA},
 }

% master thesis (as techreport and thesis)

@techreport{Petrie:1986:NAD:899644,
 author = {Petrie, Charles J.},
 title = {New Algorithms for Dependency-Directed Backtracking (Master's thesis)},
 year = {1986},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Autexas_cs%3AUTEXAS_CS%2F%2FAI86-33},
 publisher = {University of Texas at Austin},
 address = {Austin, TX, USA},
 }

@MASTERSTHESIS{Petrie:1986:NAD:12345,
 author = {Petrie, Charles J.},
 title = {New Algorithms for Dependency-Directed Backtracking (Master's thesis)},
 year = {1986},
 source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Autexas_cs%3AUTEXAS_CS%2F%2FAI86-33},
 school = {University of Texas at Austin},
 address = {Austin, TX, USA},
 }




@BOOK{book-minimal,
   author = "Donald E. Knuth",
   title = "Seminumerical Algorithms",
   publisher = "Addison-Wesley",
   year = "1981",
}

% incollection (has an editor, title, and possibly a booktitle)
@INcollection{KA:2001,
 author = {Kong, Wei-Chang},
 Title = {The implementation of electronic commerce in SMEs in Singapore (as Incoll)},
 booktitle = {E-commerce and cultural values},
 year = {2001},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}


% with bibfield 'type' before chapter (note no editor)
@INBOOK{KAGM:2001,
 author = {Kong, Wei-Chang},
 type = {Name of Chapter:},
 chapter = {The implementation of electronic commerce in SMEs in Singapore (Inbook-w-chap-w-type)},
 title = {E-commerce and cultural values},
 year = {2001},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}

%%% Notes! This is because the atsign-INBOOK citation type specifies EITHER
%%% editor or author, but not both. In my experiments with the harvard/dcu
%%% bibtex style (and presumably this applies to other styles too), bibtex
%%% ignores the editor information if author information exists in an
%%% atsign-INBOOK entry. atsign-INCOLLECTION is far more commonly used in my references,
%%% and in the absence of an editor I believe most bibtex styles will just
%%% ommit the editor from the reference - the chapter information will not
%%% end up in the in-text citation as you suggest it should be but at least
%%% there is a place to put the editor if necessary.



% was 'Inbook' -- changed to incollection - (editor is different to author) - need to tell Asad to codify as such.
@incollection{Kong:2002:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {Chapter 9},
  booktitle =   {E-commerce and cultural values (Incoll-w-text (chap 9) 'title')},
  year =        {2002},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  type =        "",
  month =       "",
  note =        "",
}

% incol when the chapter is 'text' - due to presence of editor (different to author)
@incollection{Kong:2003:IEC:887006.887011,
 author = {Kong, Wei-Chang},
 title = {The implementation of electronic commerce in SMEs in Singapore (Incoll)},
 booktitle = {E-commerce and cultural values},
 editor = {Thanasankit, Theerasak},
 year = {2003},
 isbn = {1-59140-056-2},
 pages = {51--74},
 numpages = {24},
 url = {http://portal.acm.org/citation.cfm?id=887006.887010},
 acmid = {887010},
 publisher = {IGI Publishing},
 address = {Hershey, PA, USA},
}

% ------ test
%incollection{Kong:2003:IEC:887006.887010,
% author = {Kong, Wei-Chang},
% chapter = {The implementation of electronic commerce in SMEs in Singapore (Incoll-text-in-chap)},
% booktitle = {booktitle E-commerce and cultural values},
% title =   {The title},
% editor = {Thanasankit, Theerasak},
% year = {2003},
% isbn = {1-59140-056-2},
% pages = {51--74},
% numpages = {24},
% url = {http://portal.acm.org/citation.cfm?id=887006.887010},
% acmid = {887010},
% publisher = {IGI Publishing},
% address = {Hershey, PA, USA},
%}


% ---------





% Need inbook with num in chapter

% and inbook with number in chapter
@InBook{Kong:2004:IEC:123456.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values - (InBook-num-in-chap)},
  chapter =     {9},
  year =        {2004},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  type =        "",
  month =       "",
  note =        "",
}


% and inbook with text in chapter
@Inbook{Kong:2005:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values (Inbook-text-in-chap)},
  chapter =     {The implementation of electronic commerce in SMEs in Singapore},
  year =        {2005},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  type =        {Chapter:},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  month =       "",
  note =        "",
}


% and inbook with a num and type field
@Inbook{Kong:2006:IEC:887006.887010,
  author =      {Kong, Wei-Chang},
  editor =      {Theerasak Thanasankit},
  title =       {E-commerce and cultural values (Inbook-num chap)},
  chapter =     {22},
  year =        {2006},
  address =     {Hershey, PA, USA},
  publisher =   {IGI Publishing},
  url =         {http://portal.acm.org/citation.cfm?id=887006.887010},
  type =        {Chapter (in type field)},
  pages =       {51--74},
  numpages =    {24},
  acmid =       {887010},
  isbn =        {1-59140-056-2},
  number =      "",
  month =       "",
  note =        "",
}


% and incol coz we have a BLANK chapter - due to presence of editor
%atIncollection{Kong:2006:IEC:887006.887011,
%  author =     {Kong, Wei-Chang},
%  editor =     {Theerasak Thanasankit},
%  title =      "The title"
%  booktitle =  {E-commerce and cultural values (Incol-coz-blank-chap)},
%  year =       {2006},
%  address =    {Hershey, PA, USA},
%  publisher =  {IGI Publishing},
%  url =        {http://portal.acm.org/citation.cfm?id=887006.887010},
%  type =       {Type!},
%  chapter =    {},
%  pages =      {51--74},
%  numpages =   {24},
%  acmid =      {887010},
%  isbn =       {1-59140-056-2},
%  number =     "",
%  month =      "",
%  note =       "",
%}

@article{SaeediMEJ10,
            author = {Mehdi Saeedi and Morteza Saheb Zamani and Mehdi Sedighi},
            title = {A library-based synthesis methodology for reversible logic},
            journal = {Microelectron. J.},
            volume = {41},
            number = {4},
            month = apr,
            year = {2010},
            pages = {185--194},
}

@ARTICLE{SaeediJETC10,
            author = {Mehdi Saeedi and Morteza Saheb Zamani and Mehdi Sedighi and Zahra Sasanian},
            title = {Synthesis of Reversible Circuit Using Cycle-Based Approach},
            journal = {J. Emerg. Technol. Comput. Syst.},
            volume = {6},
            number = {4},
            month = dec,
            year = {2010}
            }

% Asad's new version
@article{Kirschmer:2010:AEI:1958016.1958018,
 author = {Kirschmer, Markus and Voight, John},
 title = {Algorithmic Enumeration of Ideal Classes for Quaternion Orders},
 journal = {SIAM J. Comput.},
 issue_date = {January 2010},
 volume = {39},
 number = {5},
 month = jan,
 year = {2010},
 issn = {0097-5397},
 pages = {1714--1747},
 numpages = {34},
 url = {http://dx.doi.org/10.1137/080734467},
 doi = {https://doi.org/10.1137/080734467},
 acmid = {1958018},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
 keywords = {ideal classes, maximal orders, number theory, quaternion algebras},
}


% incol due to presence of booktitle
@incollection{Hoare:1972:CIN:1243380.1243382,
 author = {Hoare, C. A. R.},
 title = {Chapter II: Notes on data structuring},
 booktitle = {Structured programming (incoll)},
 editor = {Dahl, O. J. and Dijkstra, E. W. and Hoare, C. A. R.},
 year = {1972},
 isbn = {0-12-200550-3},
 pages = {83--174},
 numpages = {92},
 url = {http://portal.acm.org/citation.cfm?id=1243380.1243382},
 acmid = {1243382},
 publisher = {Academic Press Ltd.},
 address = {London, UK, UK},
}

% incol due to presence of booktitle
@incollection{Lee:1978:TQA:800025.1198348,
 author = {Lee, Jan},
 title = {Transcript of question and answer session},
 booktitle = {History of programming languages I (incoll)},
 editor = {Wexelblat, Richard L.},
 year = {1981},
 isbn = {0-12-745040-8},
 pages = {68--71},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/800025.1198348},
 doi = {http://doi.acm.org/10.1145/800025.1198348},
 acmid = {1198348},
 publisher = {ACM},
 address = {New York, NY, USA},
}

% incol due to booktitle
@incollection{Dijkstra:1979:GSC:1241515.1241518,
 author = {Dijkstra, E.},
 title = {Go to statement considered harmful},
 booktitle = {Classics in software engineering (incoll)},
 year = {1979},
 isbn = {0-917072-14-6},
 pages = {27--33},
 numpages = {7},
 url = {http://portal.acm.org/citation.cfm?id=1241515.1241518},
 acmid = {1241518},
 publisher = {Yourdon Press},
 address = {Upper Saddle River, NJ, USA},
}

% incol due to booktitle
@incollection{Wenzel:1992:TVA:146022.146089,
 author = {Wenzel, Elizabeth M.},
 title = {Three-dimensional virtual acoustic displays},
 booktitle = {Multimedia interface design (incoll)},
 year = {1992},
 isbn = {0-201-54981-6},
 pages = {257--288},
 numpages = {32},
 url = {http://portal.acm.org/citation.cfm?id=146022.146089},
 doi = {10.1145/146022.146089},
 acmid = {146089},
 publisher = {ACM},
 address = {New York, NY, USA},
}

% incol due to booktitle
@incollection{Mumford:1987:MES:54905.54911,
 author = {Mumford, E.},
 title = {Managerial expert systems and organizational change: some critical research issues},
 booktitle = {Critical issues in information systems research (incoll)},
 year = {1987},
 isbn = {0-471-91281-6},
 pages = {135--155},
 numpages = {21},
 url = {http://portal.acm.org/citation.cfm?id=54905.54911},
 acmid = {54911},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

@book{McCracken:1990:SSC:575315,
 author = {McCracken, Daniel D. and Golden, Donald G.},
 title = {Simplified Structured COBOL with Microsoft/MicroFocus COBOL},
 year = {1990},
 isbn = {0471514071},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

% Let's include Boris / BBeeton entries  (multi-volume works)

@book {MR781537,
    AUTHOR = {H{\"o}rmander, Lars},
     TITLE = {The analysis of linear partial differential operators. {III}},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {275},
      NOTE = {Pseudodifferential operators},
PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin, Germany},
      YEAR = {1985},
     PAGES = {viii+525},
      ISBN = {3-540-13828-5},
   MRCLASS = {35-02 (35Sxx 47G05 58G15)},
  MRNUMBER = {781536 (87d:35002a)},
MRREVIEWER = {Min You Qi},
}

@book {MR781536,
    AUTHOR = {H{\"o}rmander, Lars},
     TITLE = {The analysis of linear partial differential operators. {IV}},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {275},
      NOTE = {Fourier integral operators},
PUBLISHER = {Springer-Verlag},
   ADDRESS = {Berlin, Germany},
      YEAR = {1985},
     PAGES = {vii+352},
      ISBN = {3-540-13829-3},
   MRCLASS = {35-02 (35Sxx 47G05 58G15)},
  MRNUMBER = {781537 (87d:35002b)},
MRREVIEWER = {Min You Qi},
}

%%%%%%%%%%%%%%%%%%%%%% Start of Aptara sample bib entries




@misc{Harvard-01,
    key         = {Harvard CodeBlue},
    title       = {{CodeBlue}: Sensor Networks for Medical Care},
    note        = {http://www.eecs.harvard.edu/mdw/ proj/codeblue/},
    year        = 2008
}

@inproceedings{genre,
  title={Autoregressive Entity Retrieval},
  author={De Cao, Nicola and Izacard, Gautier and Riedel, Sebastian and Petroni, Fabio},
  booktitle={ICLR 2021-9th International Conference on Learning Representations},
  year={2021}
}
@article{de2022multilingual,
  title={Multilingual autoregressive entity linking},
  author={De Cao, Nicola and Wu, Ledell and Popat, Kashyap and Artetxe, Mikel and Goyal, Naman and Plekhanov, Mikhail and Zettlemoyer, Luke and Cancedda, Nicola and Riedel, Sebastian and Petroni, Fabio},
  journal={Transactions of the Association for Computational Linguistics},
  volume={10},
  pages={274--290},
  year={2022},
  publisher={MIT Press}
}

@inproceedings{nair2010rectified,
  title={Rectified Linear Units Improve Restricted {Boltzmann} Machines},
  author={Nair, Vinod and Hinton, Geoffrey E.},
  booktitle={International conference on machine learning},
  year={2010},
  pages={807–814},

}


@inproceedings{msmarco,
  author    = {Tri Nguyen and
               Mir Rosenberg and
               Xia Song and
               Jianfeng Gao and
               Saurabh Tiwary and
               Rangan Majumder and
               Li Deng},
  title     = {{MS} {MARCO:} {a} Human Generated MAchine Reading COmprehension Dataset},
  booktitle    = {Proceedings of the Workshop on Cognitive Computation: Integrating neural and symbolic approaches 2016 co-located with the 30th Annual Conference on Neural Information Processing Systems},
year      = {2016},
}


@inproceedings{clarke2009overviewclueweb,
  title={Overview of the {TREC} 2009 Web Track},
  author={Clarke, Charles L.A. and Craswell, Nick and Soboroff, Ian},
  year={2010},
  booktitle    = {Proceedings of The Eighteenth Text REtrieval Conference},
  series       = {{NIST} Special Publication},
  volume       = {500-278},
}
@inproceedings{clarke2004overviewGov,
  title={Overview of the {TREC} 2004 Terabyte Track},
  author={Clarke, Charles L.A. and Craswell, Nick and Soboroff, Ian},
  booktitle    = {Proceedings of the Thirteenth Text REtrieval Conference},
  series       = {{NIST} Special Publication},
  volume       = {500-261},
  year={2004}
}

@article{qin2013introducingmq,
  title={Introducing LETOR 4.0 datasets},
  author={Qin, Tao and Liu, Tie-Yan},
  journal={arXiv preprint arXiv:1306.2597},
  year={2013}
}

@inproceedings{chen2023understanding,
      title={Understanding Differential Search Index for Text Retrieval}, 
      author={Xiaoyang Chen and Yanjiang Liu and Ben He and Le Sun and Yingfei Sun},
      year={2023},
      pages        = {10701--10717},
      booktitle={Findings of the Association for Computational Linguistics},
}
@inproceedings{shah2022situating,
  title={Situating Search},
  author={Shah, Chirag and Bender, Emily M},
  booktitle={ACM SIGIR Conference on Human Information Interaction and Retrieval},
  pages={221--232},
  year={2022}
}
@inproceedings{zhuang2021deep,
  title={Deep Query Likelihood Model for Information Retrieval},
  author={Zhuang, Shengyao and Li, Hang and Zuccon, Guido},
  booktitle={Advances in Information Retrieval: 43rd European Conference on IR Research, ECIR 2021, Virtual Event, March 28--April 1, 2021, Proceedings, Part II 43},
  pages={463--470},
  year={2021},
  organization={Springer}
}

@inproceedings{tang2021improving,
  title={Improving Document Representations by Generating Pseudo Query Embeddings for Dense Retrieval},
  author={Tang, Hongyin and Sun, Xingwu and Jin, Beihong and Wang, Jingang and Zhang, Fuzheng and Wu, Wei},
  booktitle={Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={5054--5064},
  year={2021}
}
@article{herbrich1999support,
  title={Support vector learning for ordinal regression},
  author={Herbrich, Ralf and Graepel, Thore and Obermayer, Klaus},
  year={1999},
  publisher={IET}
}

@article{freund2003efficient,
  title={An efficient boosting algorithm for combining preferences},
  author={Freund, Yoav and Iyer, Raj and Schapire, Robert E and Singer, Yoram},
  journal={Journal of machine learning research},
  volume={4},
  number={Nov},
  pages={933--969},
  year={2003}
}

@inproceedings{burges2005learning,
  title={Learning to Rank Using Gradient Descent},
  author={Burges, Chris and Shaked, Tal and Renshaw, Erin and Lazier, Ari and Deeds, Matt and Hamilton, Nicole and Hullender, Greg},
  booktitle={Proceedings of the 22nd international conference on Machine learning},
  pages={89--96},
  year={2005}
}

@inproceedings{cao2007learning,
  title={Learning to Rank: from Pairwise Approach to Listwise Approach},
  author={Cao, Zhe and Qin, Tao and Liu, Tie-Yan and Tsai, Ming-Feng and Li, Hang},
  booktitle={Proceedings of the 24th international conference on Machine learning},
  pages={129--136},
  year={2007}
}
@inproceedings{xia2008listwise,
  title={Listwise Approach to Learning to Rank: Theory and Algorithm},
  author={Xia, Fen and Liu, Tie-Yan and Wang, Jue and Zhang, Wensheng and Li, Hang},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={1192--1199},
  year={2008}
}
@inproceedings{khosla2020supervised,
  title={Supervised Contrastive Learning},
  author={Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  booktitle={Advances in neural information processing systems},
  volume={33},
  pages={18661--18673},
  year={2020}
}
@inproceedings{tian2020makes,
  title={What Makes for Good Views for Contrastive Learning?},
  author={Tian, Yonglong and Sun, Chen and Poole, Ben and Krishnan, Dilip and Schmid, Cordelia and Isola, Phillip},
  booktitle={Advances in neural information processing systems},
  volume={33},
  pages={6827--6839},
  year={2020}
}



@article{craswell2020overviewtrec2019,
  title={Overview of the {TREC} 2019 deep learning track},
  author={Craswell, Nick and Mitra, Bhaskar and Yilmaz, Emine and Campos, Daniel and Voorhees, Ellen M},
  journal={arXiv preprint arXiv:2003.07820},
  year={2020}
}
@inproceedings{bm25,
  title={Okapi at {TREC}-3},
  author={Robertson, Stephen E. and Walker, Steve and Jones, Susan and Hancock-Beaulieu, Micheline M. and Gatford, Mike},
  year={1994},
  booktitle    = {Proceedings of The Third Text REtrieval Conference},
  series       = {{NIST} Special Publication},
  volume       = {500-225},
  pages        = {109--126},
}
@article{hiemstra2000probabilistic,
  title={A Probabilistic Justification for Using tf$\times$idf Term Weighting in Information Retrieval},
  author={Hiemstra, Djoerd},
  journal={International Journal on Digital Libraries},
  year={2000},
  volume = 3,
  publisher={Springer}
}
@article{salton1988term,
  title={Term-weighting Approaches in Automatic Text Retrieval},
  author={Salton, Gerard and Buckley, Christopher},
  journal={Information Processing \& Management},
  year={1988},
  publisher={Elsevier}
}
@inproceedings{pipeline2,
  title={Learning Term Discrimination},
  author={Frej, Jibril and Mulhem, Philippe and Schwab, Didier and Chevallet, Jean-Pierre},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages = {1993--1996},
  year={2020}
}
@inproceedings{deepTR,
  title={Learning to Reweight Terms with Distributed Representations},
  author={Zheng, Guoqing and Callan, Jamie},
  booktitle={Proceedings of the 2015 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages = {575–584},
  year={2015}
}

@inproceedings{ganguly2015word,
  title={Word Embedding Based Generalized Language Model for Information Retrieval},
  author={Ganguly, Debasis and Roy, Dwaipayan},
  booktitle={Proceedings of the 2015 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2015}
}

@article{deepCT,
  title={Context-aware sentence/passage term importance estimation for first stage retrieval},
  author={Dai, Zhuyun and Callan, Jamie},
  journal={arXiv preprint arXiv:1910.10687},
  year={2019}
}
@article{bai2020sparterm,
  title={SparTerm: Learning Term-based Sparse Representation for Fast Text Retrieval},
  author={Bai, Yang and Li, Xiaoguang and Wang},
  journal={arXiv preprint arXiv:2010.00768},
  year={2020}
}
@inproceedings{zhao2010term,
  title={Term Necessity Prediction},
  author={Zhao, Le and Callan, Jamie},
  booktitle    = {Proceedings of the 19th {ACM} Conference on Information and Knowledge Management},
pages        = {259--268},

  year={2010}
}
@article{furnas1987vocabulary,
  title={The Vocabulary Problem in Human-system Communication},
  author={Furnas, George W. and Landauer, Thomas K. and Gomez, Louis M. and Dumais, Susan, T.},
  journal={Communications of the ACM},
  year={1987},
  publisher={ACM},
  pages = {964--971},
  volume = 30,
  issue = 11,
}
@article{zhan2020repbert,
  title={{RepBERT}: Contextualized Text Embeddings for First-stage Retrieval},
  author={Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Zhang, Min and Ma, Shaoping},
  journal={arXiv preprint arXiv:2006.15498},
  year={2020}
}
@inproceedings{karpukhin2020dense,
  title={Dense Passage Retrieval for Open-domain Question Answering},
  author={Karpukhin, Vladimir and O{\u{g}}uz, Barlas and Min, Sewon and Lewis, Patrick and Wu},
  booktitle={Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing},
  pages        = {6769--6781},
  year={2020}
}
@inproceedings{attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  year={2017}
}



@article{luan2021sparse,
  title={Sparse, Dense, and Attentional Representations for Text Retrieval},
  author = {Luan, Yi  and
      Eisenstein, Jacob  and
      Toutanova, Kristina},
  journal = {TACL},
  year={2021},
}
@inproceedings{datar2004locality,
  title={Locality-sensitive hashing scheme based on p-stable distributions},
  author={Datar, Mayur and Immorlica},
  year={2004}
}
@article{bentley1975multidimensional,
  title={Multidimensional Binary Search Trees Used for Associative Searching},
  author={Bentley, Jon Louis},
  journal={Communications of the ACM},
  volume={18},
  number={9},
  pages={509--517},
  year={1975},
  publisher={ACM New York, NY, USA}
}
@inproceedings{beis1997shape,
  title={Shape Indexing Using Approximate Nearest-neighbour Search in High-dimensional Spaces},
  author={Beis, Jeffrey S. and Lowe, David G.},
  booktitle={Proceedings of IEEE computer society conference on computer vision and pattern recognition},
  year={1997},
  pages = {1000-1006}
}
@inproceedings{nie2020dc,
  title={DC-BERT: Decoupling Question and Document for Efficient Contextual Encoding},
  author={Nie, Ping and Zhang, Yuyu and Geng, Xiubo and Ramamurthy, Arun and Song, Le and Jiang, Daxin},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2020},
  pages = {1829--1832},
  publisher = {ACM}
}
@inproceedings{khattab2020colbert,
  title={{ColBERT}: Efficient and Effective Passage Search via Contextualized Late Interaction over {BERT}},
  author={Khattab, Omar and Zaharia, Matei},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2020},
  pages = {39-48}
}
@inproceedings{macavaney2020efficient,
  title = {Efficient Document Re-Ranking for Transformers by Precomputing Term Representations},
  author = {MacAvaney, Sean and Nardini, Franco Maria and Perego, Raffaele and Tonellotto, Nicola and Goharian, Nazli and Frieder, Ophir},
  booktitle = {Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2020}
}
@inproceedings{clinchant2013aggregating,
  title={Aggregating Continuous Word Embeddings for Information Retrieval},
  booktitle = {Proceedings of the Workshop on Continuous Vector Space Models and their Compositionality},
  author={Clinchant, St{\'e}phane and Perronnin, Florent},
  year={2013}
}
@article{probability,
  title={Relevance Weighting of Search Terms},
  author={Robertson, Stephen E. and Spärck Jones, Karen},
  journal={Journal of the American Society for Information Science},
  year={1976},
}
@article{robertson2009probabilistic,
  title={The Probabilistic Relevance Framework: BM25 and Beyond},
  author={Robertson, Stephen E},
  year={2009},
  journal={Foundations and Trends in Information Retrieval},
}

@article{ji2022survey,
  title={Survey of Hallucination in Natural Language Generation},
  author={Ji, Ziwei and Lee, Nayeon and Frieske, Rita and Yu, Tiezheng and Su, Dan and Xu, Yan and Ishii, Etsuko and Bang, Yejin and Madotto, Andrea and Fung, Pascale},
  journal={ACM Computing Surveys},
  year={2023},
  volume = 55,
  pages = {Article 248},
}
@article{chen2020customizablelongtext,
  title={Customizable Text Generation via Conditional Text Generative Adversarial Network},
  author={Chen, Jinyin and Wu, Yangyang and Jia, Chengyu and Zheng, Haibin and Huang, Guohan},
  journal={Neurocomputing},
  volume={416},
  year={2020},
  publisher={Elsevier}
}

@article{van1977theoretical,
  title={A theoretical basis for the use of co-occurrence data in information retrieval},
  author={van Rijsbergen, Cornelis Joost},
  journal={Journal of documentation},
  year={1977},
  publisher={MCB UP Ltd}
}

@inproceedings{dai2018convolutional,
  title={Convolutional Neural Networks for Soft-matching n-grams in Ad-hoc Search},
  author={Dai, Zhuyun and Xiong, Chenyan and Callan, Jamie and Liu, Zhiyuan},
  booktitle={WSDM},
  year={2018}
}
@inproceedings{guo2019matchzoo,
  title={Matchzoo: A learning, practicing, and developing system for neural text matching},
  author={Guo, Jiafeng and Fan, Yixing and Ji, Xiang and Cheng, Xueqi},
  booktitle={Proceedings of the 2019 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={1297--1300},
  year={2019}
}
@inproceedings{guo2016deep,
  title={A Deep Relevance Matching Model for Ad-hoc Retrieval},
  author={Guo, Jiafeng and Fan, Yixing and Ai, Qingyao and Croft, W Bruce},
  booktitle={Proceedings of the 25th ACM international on conference on information and knowledge management},
  pages={55--64},
  year={2016},
  publisher = {ACM}
}
@inproceedings{huang2013learning,
  title={Learning deep structured semantic models for web search using clickthrough data},
  author={Huang, Po-Sen and He, Xiaodong},
  booktitle={ACM CIKM},
  year={2013}
}
@inproceedings{DBLP:journals/corr/abs-1802-05365elmo,
  author    = {Matthew E. Peters and
               Mark Neumann and
               Mohit Iyyer and
               Matt Gardner and
               Christopher Clark and
               Kenton Lee and
               Luke Zettlemoyer},
  title     = {Deep Contextualized Word Representations},
  booktitle = {ACL},
  year      = {2018},
  pages = {2227--2237},
}
@inproceedings{bert,
  title={{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  year={2019},
  booktitle={Proceedings of NAACL-HLT},
}


@inproceedings{lee2023nonparametric,
  title={Nonparametric Decoding for Generative Retrieval},
  author={Lee, Hyunji and Kim, Jaeyoung and Chang, Hoyeon and Oh, Hanseok and Yang, Sohee and Karpukhin, Vladimir and Lu, Yi and Seo, Minjoon},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2023},
  pages={12642--12661},
  year={2023}
}


@article{chang2020pre,
  title={Pre-training Tasks for Embedding-based Large-scale Retrieval},
  author={Chang, Wei-Cheng and Yu},
  journal={arXiv preprint arXiv:2002.03932},
  year={2020}
}
@inproceedings{lee2019latent,
  title={Latent Retrieval for Weakly Supervised Open Domain Question Answering},
  author={Lee, Kenton and Chang, Ming-Wei and Toutanova, Kristian},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages = {6086--6096},
  year={2019}
}
@inproceedings{ma2021pre,
  title = {Pre-Training for Ad-Hoc Retrieval: Hyperlink is Also You Need},
  author = {Ma, Zhengyi and Dou, Zhicheng and Xu, Wei and Zhang, Xinyu and Jiang, Hao and Cao, Zhao and Wen, Ji-Rong},
  booktitle={Proceedings of the 30th ACM International Conference on Information \& Knowledge Management},
  year={2021},
  publisher = {ACM}
}
@article{liu2019roberta,
  title={Roberta: A robustly optimized {BERT} pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}
@inproceedings{markedbert,
  title={{MarkedBERT}: Integrating Traditional {IR} Cues in Pre-trained Language Models for Passage Retrieval},
  author={Boualili, Lila and Moreno, Jose G. and Boughanem, Mohand},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2020}
}
@inproceedings{prop,
  title={PROP: Pre-Training with Representative Words Prediction for Ad-Hoc Retrieval},
  author={Ma, Xinyu and Guo, Jiafeng and Zhang, Ruqing and Fan, Yixing and Ji, Xiang and Cheng, Xueqi},
  booktitle={Proceedings of the 14th ACM international conference on web search and data mining},
  pages={283--291},
  year={2021},
}
@article{LTR1,
  title={Learning to Rank for Information Retrieval},
  author={Liu, Tie-Yan},
  journal={Foundations and Trends in Information Retrieval},
  volume={3},
  number={3},
  pages={225--331},
  year={2009},
  publisher={Now Publishers, Inc.}
}
@article{LTR2,
  title={Learning to Rank for Information Retrieval and Natural Language Processing},
  author={Li, Hang},
  journal={Synthesis Lectures on Human Language Technologies},
  year={2014}
}
@article{naturalquestion,
  title={Natural Questions: a Benchmark for Question Answering Research},
  author = {Kwiatkowski, Tom  and
      Palomaki, Jennimaria  and
      Redfield, Olivia  and
      Collins, Michael  and
      Parikh, Ankur},
  journal={Transactions oof the Association for Computational Linguistics},
  volume = 7,
  pages = {452--466},
  year={2019},
}
@inproceedings{NCI,
  title={A Neural Corpus Indexer for Document Retrieval},
  author={Wang, Yujing and Hou, Yingyan and Wang, Haonan and Miao, Ziming and
  Wu, Shibin and Sun, Hao and Chen, Qi and Xia, Yuqing and Chi, Chengmin and Zhao, Guoshuai and Liu, Zheng and Xie, Xing and Sun, Hao and Deng, Weiwei and Zhang, Qi and Yang, Mao},
  booktitle={Advances in neural information processing systems},
  pages={25600--25614},
  year={2022}
}
@article{modelBased,
    author = {Metzler, Donald and Tay, Yi and Bahri, Dara and Najork, Marc},
    title = {Rethinking Search: Making Domain Experts out of Dilettantes},
    year = {2021},
    journal = {ACM SIGIR Forum},
    volume = 55,
    pages = {Article 13}
}

@inproceedings{DSI,
  title={Transformer Memory as a Differentiable Search Index},
  author={Tay, Yi and Tran, Vinh Q and Dehghani, Mostafa and Ni, Jianmo and Bahri, Dara},
  booktitle={Advances in neural information processing systems},
  pages={21831--21843},

  year={2022}
}

@inproceedings{seal,
  title={Autoregressive Search Engines: Generating Substrings as Document Identifiers},
  author={Bevilacqua, Michele and Ottaviano, Giuseppe and Lewis, Patrick and Yih, Wen-tau and Riedel, Sebastian and Petroni, Fabio},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022}
}

@inproceedings{chen2022corpusbrain,
  title={CorpusBrain: Pre-train a Generative Retrieval Model for Knowledge-Intensive Language Tasks},
  author={Chen, Jiangui and Zhang, Ruqing and Guo, Jiafeng and Liu, Yiqun and Fan, Yixing and Cheng, Xueqi},
  booktitle={Proceedings of the 31st ACM International Conference on Information \& Knowledge Management},
  year={2022},
  pages = {191-200}
}


@article{johnson2019billionbertANN,
  title={Billion-scale similarity search with gpus},
  author={Johnson, Jeff and Douze, Matthijs and J{\'e}gou, Herv{\'e}},
  journal={IEEE Transactions on Big Data},
  volume={7},
  number={3},
  pages={535--547},
  year={2019},
  publisher={IEEE}
}
@misc{doct5query,
  title={From Doc2query to DocTTTTTquery},
  author={Nogueira, Rodrigo and Lin, Jimmy},
  howpublished={An MS MARCO Passage Retrieval Task Publication},
  month={12},
  year={2019},
  note = {University of Waterloo},
}
@article{zhang2021adversarialar2,
  title={Adversarial retriever-ranker for dense text retrieval},
  author={Zhang, Hang and Gong, Yeyun and Shen, Yelong and Lv, Jiancheng and Duan, Nan and Chen, Weizhu},
  journal={arXiv preprint arXiv:2110.03611},
  year={2021}
}
@article{gao2021unsupervisedcocondenser,
  title={Unsupervised corpus aware language model pre-training for dense passage retrieval},
  author={Gao, Luyu and Callan, Jamie},
  journal={arXiv preprint arXiv:2108.05540},
  year={2021}
}
@inproceedings{application1,
  title={Cascade Ranking for Operational E-commerce Search},
  author={Liu, Shichen and Xiao, Fei and Ou, Wenwu and Si, Luo},
  booktitle={SIGKDD},
  year={2017},
  pages = {1557–1565},
  publisher = {ACM}
}
@inproceedings{application2,
  title={Query Understanding at Bing},
  author={Pedersen, Jan},
  booktitle = {SIGIR Industry Track},
  year={2010}
}
@article{application3,
  title={Answering English questions by computer: a survey},
  author={Simmons, Robert F.},
  journal = {Commnunications of the ACM},
  volume = {8},
  issue = {1},
  pages = {53--70},
  year={1965},
}
@inproceedings{pipeline1,
  title={Context-aware Term Weighting for First Stage Passage Retrieval},
  author={Dai, Zhuyun and Callan, Jamie},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2020},
  pages = {1533--1536},
  publisher = {ACM}
}

@inproceedings{pipeline4,
  title={Optimizing Dense Retrieval Model Training with Hard Negatives},
  author={Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Guo, Jiafeng and Zhang, Min and Ma, Shaoping},
  booktitle={Proceedings of the 2020 ACM SIGIR International Conference on Theory of Information Retrieval},
year={2020}

}
@inproceedings{sun2020colakewikiextractor,
  title={Colake: Contextualized Language and Knowledge Embedding},
  author={Sun, Tianxiang and Shao, Yunfan},
  booktitle={COLING},
  year={2020}
}


@inproceedings{zhang2022use,
  title={Use All The Labels: A Hierarchical Multi-Label Contrastive Learning Framework},
  author={Zhang, Shu and Xu, Ran and Xiong, Caiming and Ramaiah, Chetan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages        = {16639--16648},
  year={2022}
}
@inproceedings{bi2021askingbik,
  title={Asking Clarifying Questions Based on Negative Feedback in Conversational Search},
  author={Bi, Keping and Ai, Qingyao and Croft, W Bruce},
  booktitle={Proceedings of the 2021 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={157--166},
  year={2021}
}

@inproceedings{giunchiglia2020coherent,
  title={Coherent Hierarchical Multi-label Classification Networks},
  author={Giunchiglia, Eleonora and Lukasiewicz, Thomas},
  booktitle={Advances in neural information processing systems},
  pages={9662--9673},
  year={2020},
}


@article{zhou2022ultron,
  title={Ultron: An Ultimate Retriever on Corpus with a Model-based Indexer},
  author={Zhou, Yujia and Yao, Jing and Dou, Zhicheng and Wu, Ledell and Zhang, Peitian and Wen, Ji-Rong},
  journal={arXiv preprint arXiv:2208.09257},
  year={2022}
}

@inproceedings{kikuchi2016controlling,
  title={Controlling Output Length in Neural Encoder-decoders},
  author={Kikuchi, Yuta and Neubig, Graham and Sasano, Ryohei and Takamura, Hiroya and Okumura, Manabu},
booktitle = "EMNLP",
  year={2016}
}
@inproceedings{zhuang2022bridgingdsiqg,
  title={Bridging the Gap between Indexing and Retrieval for Differentiable Search Index with Query Generation},
  author={Zhuang, Shengyao and Ren, Houxing and Shou, Linjun},
  booktitle={Gen-IR@SIGIR 2023: The First Workshop on Generative Information Retrieval},
  year={2022}
}
@inproceedings{xiong2020approximate,
  title={Approximate Nearest Neighbor Negative Contrastive Learning for Dense Text Retrieval},
  author={Xiong, Lee and Xiong, Chenyan and Li, Ye and Tang, Kwok-Fung and Liu, Jialin and Bennett, Paul N and Ahmed, Junaid and Overwijk, Arnold},
  booktitle={International Conference on Learning Representations},
  year={2020}
}
@incollection{ricci2011introductionndcg,
  title={Introduction to Recommender Systems Handbook},
  author={Ricci, Francesco and Rokach, Lior and Shapira, Bracha},
  booktitle={Recommender Systems Handbook},
  year={2011},
  publisher={Springer}
}
@article{fuhr2008probability,
  title={A probability ranking principle for interactive information retrieval},
  author={Fuhr, Norbert},
  journal={Information Retrieval},
  volume={11},
  number={3},
  pages={251--265},
  year={2008},
  publisher={Springer}
}
@inproceedings{scholer2011quantifying,
  title={Quantifying Test Collection Quality Based on the Consistency of Relevance Judgements},
  author={Scholer, Falk and Turpin, Andrew and Sanderson, Mark},
  booktitle={Proceedings of the 2011 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2011},
}

@article{2020Beam,
  title={Beam Search Algorithm for Anti-Collision Trajectory Planning for Many-to-Many Encounter Situations with Autonomous Surface Vehicles},
  author={Koszelew, Jolanta  and  Karbowska-Chilinska, Joanna},
  journal={Sensors},
  volume={20},
  year={2020},
  issue = {15},
  pages = {4115}
}
@inproceedings{2022Traininggpt,
  title={Training Language Models to Follow Instructions with Human Feedback},
  author={Ouyang, Long and Wu, Jeff and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll L. and Mishkin},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022},
}
@article{1998Ateacher,
  title={A Learning Algorithm for Continually Running Fully Recurrent Neural Networks},
  author={Williams, Ronald J. and  Zipser, David},
  journal={Neural Computation},
  year={1998},
  volume = {1},
  pages = {270-280},
}
@article{1995Inverted,
  title={Inverted File Partitioning Schemes in Multiple Disk Systems},
  author={Jeong, Byeong-Soo},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  year={1995},
}
@inproceedings{voorhees2004overviewrobust,
  title={Overview of the {TREC} 2004 Robust Retrieval Track.},
  author={Voorhees, Ellen M},
  booktitle={TREC},
  pages={69--77},
  year={2004}
}
@inproceedings{dai2019deepermetric,
  title={Deeper text understanding for IR with contextual neural language modeling},
  author={Dai, Zhuyun and Callan, Jamie},
  booktitle={Proceedings of the 2019 ACM SIGIR International Conference on Theory of Information Retrieval}, 
  year={2019}
}
@inproceedings{macavaney2019cedrmetric,
  title={CEDR: Contextualized embeddings for document ranking},
  author={MacAvaney, Sean and Yates, Andrew and Cohan, Arman and Goharian, Nazli},
  booktitle={Proceedings of the 2019 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2019}
}
@article{guo2022semanticpipeline5,
  title={Semantic models for the first-stage retrieval: A comprehensive review},
  author={Guo, Jiafeng and Cai, Yinqiong and Fan, Yixing and Sun, Fei and Zhang, Ruqing and Cheng, Xueqi},
  journal={ACM Transactions on Information Systems (TOIS)},
  year={2022},
  publisher={ACM New York, NY}
}
@inproceedings{luo2022studyhardindex,
  title={A Study on the Efficiency and Generalization of Light Hybrid Retrievers},
  author={Luo, Man and Jain, Shashank and Gupta, Anchit and Einolghozati, Arash and Oguz, Barlas and Chatterjee, Debojeet and Chen, Xilun and Baral, Chitta and Heidari, Peyman},
  journal={SpaNLP ACL 2022 Workshop},
  year={2022}
}
@inproceedings{zhan2021jointlyjpq,
  title={Jointly optimizing query encoder and product quantization to improve retrieval performance},
  author={Zhan, Jingtao and Mao, Jiaxin and Liu, Yiqun and Guo, Jiafeng and Zhang, Min and Ma, Shaoping},
  booktitle={CIKM},
  pages={2487--2496},
  year={2021}
}
@inproceedings{robertson2010extending,
  title={Extending average precision to graded relevance judgments},
  author={Robertson, Stephen E and Kanoulas, Evangelos and Yilmaz, Emine},
  booktitle={Proceedings of the 33rd international ACM SIGIR conference on Research and development in information retrieval},
  pages={603--610},
  year={2010}
}
@article{ferrante2020interval,
  title={How do interval scales help us with better understanding IR evaluation measures?},
  author={Ferrante, Marco and Ferro, Nicola and Losiouk, Eleonora},
  journal={Information Retrieval Journal},
  volume={23},
  pages={289--317},
  year={2020},
  publisher={Springer}
}
@article{nogueira2019multi,
  title={Multi-stage document ranking with BERT},
  author={Nogueira, Rodrigo and Yang, Wei and Cho, Kyunghyun and Lin, Jimmy},
  journal={arXiv preprint arXiv:1910.14424},
  year={2019}
}
@inproceedings{he-etal-2018-dureader,
    title = "{D}u{R}eader: a {C}hinese Machine Reading Comprehension Dataset from Real-world Applications",
    author = "He, Wei  and
      Liu, Kai  and
      Liu, Jing  and
      Lyu, Yajuan  and
      Zhao, Shiqi  and
      Xiao, Xinyan  and
      Liu, Yuan  and
      Wang, Yizhong  and
      Wu, Hua  and
      She, Qiaoqiao  and
      Liu, Xuan  and
      Wu, Tian  and
      Wang, Haifeng",
  booktitle={Proceedings of the Workshop on Machine Reading for Question Answering},
  pages        = {37--46},
  year         = {2018},
}

@inproceedings{lu-etal-2021-lessismore,
    title = "Less is More: Pretrain a Strong {S}iamese Encoder for Dense Text Retrieval Using a Weak Decoder",
    author = "Lu, Shuqi  and
      He, Di  and
      Xiong, Chenyan  and
      Ke, Guolin  and
      Malik, Waleed  and
      Dou, Zhicheng  and
      Bennett, Paul  and
      Liu, Tie-Yan  and
      Overwijk, Arnold",
  booktitle={Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages        = {2780--2791},
    year = "2021",
}
@inproceedings{10.1145/3477495.3531772costa,
author = {Ma, Xinyu and Guo, Jiafeng and Zhang, Ruqing and Fan, Yixing and Cheng, Xueqi},
title = {Pre-Train a Discriminative Text Encoder for Dense Retrieval via Contrastive Span Prediction},
year = {2022},
pages        = {848--858},
booktitle = {Proceedings of the 2022 ACM SIGIR International Conference on Theory of Information Retrieval},
}
@inproceedings{khosla2020supervisedce,
  title={Supervised Contrastive Learning},
  author={Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  booktitle={Advances in neural information processing systems},
  year={2020}
}
@inproceedings{hoffmann2022rankingce,
  title={Ranking Info Noise Contrastive Estimation: Boosting Contrastive Learning via Ranked Positives},
  author={Hoffmann, David T and Behrmann, Nadine and Gall, Juergen and Brox, Thomas and Noroozi, Mehdi},
  booktitle={AAAI Conference on Artificial Intelligence},
  year={2022}
}
@inproceedings{10.1145/1651318.1651328pubmed,
author = {Yu, Hwanjo and Kim, Taehoon and Oh, Jinoh and Ko, Ilhwan and Kim, Sungchul and Han, Wook-Shin},
title = {Enabling Multi-Level Relevance Feedback on {Pubmed} by Integrating Rank Learning into {DBMS}},
year = {2009},
booktitle={Proceedings of the third international workshop on Data and text mining in bioinformatics},
}
@inproceedings{scheel11arec,
author = {Scheel, Christian and Lommatzsch, Andreas and Albayrak, Sahin},
title = {Performance Measures for Multi-Graded Relevance},
  booktitle={Proceedings of the Second International Conference on Semantic Personalized Information Management: Retrieval and Recommendation-Volume 781},
year = {2011},
}
@InProceedings{10.1007/978-3-540-31871-2_22ntcir,
author="Sakai, Tetsuya",
editor="Myaeng, Sung Hyon
and Zhou, Ming
and Wong, Kam-Fai
and Zhang, Hong-Jiang",
title="Ranking the {NTCIR} Systems Based on Multigrade Relevance",
booktitle="Information Retrieval Technology",
year="2005",
publisher="Springer Berlin Heidelberg",
}
@inproceedings{10.1145/1273496.1273513listnet,
author = {Cao, Zhe and Qin, Tao and Liu, Tie-Yan and Tsai, Ming-Feng and Li, Hang},
title = {Learning to Rank: From Pairwise Approach to Listwise Approach},
year = {2007},
isbn = {9781595937933},
booktitle={International conference on machine learning},
}

@inproceedings{10.1145/3269206.3271784lambdaloss,
author = {Wang, Xuanhui and Li, Cheng and Golbandi, Nadav and Bendersky, Michael and Najork, Marc},
title = {The LambdaLoss Framework for Ranking Metric Optimization},
year = {2018},
booktitle    = {Proceedings of the 27th {ACM} International Conference on Information and Knowledge Management},
pages        = {1313--1322},
}
@article{burges2010ranknet,
  title={From {Ranknet} to {Lambdarank} to {Lambdamart}: An Overview},
  author={Burges, Christopher JC},
  journal={Learning},
  volume={11},
  number={23-581},
  pages={81},
  year={2010}
}
@article{jarvelin2002cumulatedndcg,
  title={Cumulated Gain-based Evaluation of {IR} Techniques},
  author={J{\"a}rvelin, Kalervo and Kek{\"a}l{\"a}inen, Jaana},
  journal={ACM Transactions on Information Systems},
  year={2002},
  volume = {20},
  pages = {422-446},
  publisher={ACM New York, NY, USA}
}
@inproceedings{jarvelin2008discountednsdcg,
  title={Discounted cumulated gain based evaluation of multiple-query IR sessions},
  author={J{\"a}rvelin, Kalervo and Price, Susan L and Delcambre, Lois ML and Nielsen, Marianne Lykke},
  booktitle={European Conference on Information Retrieval},
  pages={4--15},
  year={2008},
  organization={Springer}
}
@article{chapelle2011intentERR,
  title={Intent-based Diversification of Web Search Results: {Metrics} and Algorithms},
  author={Chapelle, Olivier and Ji, Shihao and Liao, Ciya and Velipasaoglu, Emre and Lai, Larry and Wu, Su-Lin},
  journal={Information Retrieval},
  year={2011},
  volume = {14}, 
  pages = {572–592},
  publisher={Springer}
}
@inproceedings{10.1145/1645953.1646033ERRori,
author = {Chapelle, Olivier and Metlzer, Donald and Zhang, Ya and Grinspan, Pierre},
title = {Expected Reciprocal Rank for Graded Relevance},
year = {2009},
isbn = {9781605585123},
booktitle = {Proceedings of the 18th ACM conference on Information and knowledge management},
}
@article{van2008visualizingtsne,
  title={Visualizing Data Using {T-SNE}.},
  author={van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of Machine Learning Research},
  volume={9},
  number={11},
  year={2008}
}
@inproceedings{chapelle2011yahoo,
  title={Yahoo! {Learning} to Rank Challenge Overview},
  author={Chapelle, Olivier and Chang, Yi},
  booktitle={Proceedings of the Learning to Rank Challenge},
  pages={1--24},
  year={2011},
  organization={PMLR}
}
@inproceedings{sakai2011usingyahooqa,
  title={Using graded-relevance metrics for evaluating community QA answer selection},
  author={Sakai, Tetsuya and Ishikawa, Daisuke and Kando, Noriko and Seki, Yohei and Kuriyama, Kazuko and Lin, Chin-Yew},
  booktitle={Proceedings of the fourth ACM international conference on Web search and data mining},
  pages={187--196},
  year={2011}
}
@article{radford2018improvinggpt,
  title={Improving language understanding by generative pre-training},
  author={Radford, Alec and Narasimhan, Karthik and Salimans, Tim and Sutskever, Ilya and others},
  year={2018},
  publisher={OpenAI}
}
@inproceedings{dietz2017treccar,
  title={{TREC} Complex Answer Retrieval Overview.},
  author={Dietz, Laura and Verma, Manisha and Radlinski, Filip and Craswell, Nick},
  booktitle={TREC},
  year={2017}
}
@inproceedings{10.1145/3289600.3291006wassrank,
author = {Yu, Hai-Tao and Jatowt, Adam and Joho, Hideo and Jose, Joemon M. and Yang, Xiao and Chen, Long},
title = {WassRank: Listwise Document Ranking Using Optimal Transport Theory},
year = {2019},
booktitle = {WSDM},

}
@inproceedings{10.1145/775047.775067optimizing,
author = {Joachims, Thorsten},
title = {Optimizing Search Engines Using Clickthrough Data},
year = {2002},
isbn = {158113567X},
booktitle = {KDD},
}
@inproceedings{montanes2011improvingbinary,
  title={Improving Stacking Approach for Multi-label Classification},
  author={Monta{\~n}{\'e}s, Elena and Quevedo, Jos{\'e} Ram{\'o}n and del Coz, Juan Jos{\'e}},
  booktitle={Proceedings of the 2011 Spanish Conference on Artificial Intelligence},
  pages={484--500},
  year={2011}
}
@inproceedings{10.1145/1390334.1390446binary1,
author = {Clarke, Charles L.A. and Kolla, Maheedhar and Cormack, Gordon V. and Vechtomova, Olga and Ashkan, Azin and B\"{u}ttcher, Stefan and MacKinnon, Ian},
title = {Novelty and Diversity in Information Retrieval Evaluation},
year = {2008},
pages        = {659--666},
isbn = {9781605581644},
booktitle = {Proceedings of the 2008 ACM SIGIR International Conference on Theory of Information Retrieval},
}
@inproceedings{10.1145/1571941.1571963binary2,
author = {Wang, Jun and Zhu, Jianhan},
title = {Portfolio Theory of Information Retrieval},
year = {2009},
booktitle = {Proceedings of the 2009 ACM SIGIR International Conference on Theory of Information Retrieval},
}
@article{SPINK1998599multi,
title = {From highly relevant to not relevant: examining different regions of relevance},
journal = {Information Processing & Management},
volume = {34},
number = {5},
pages = {599-621},
year = {1998},
issn = {0306-4573},
doi = {https://doi.org/10.1016/S0306-4573(98)00025-9},
url = {https://www.sciencedirect.com/science/article/pii/S0306457398000259},
author = {Amanda Spink and Howard Greisdorf and Judy Bateman},
}
@inproceedings{Lewis2019BARTDS,
  title={{BART}: Denoising Sequence-to-Sequence Pre-training for Natural Language Generation, Translation, and Comprehension},
  author={Mike Lewis and Yinhan Liu and Naman Goyal and Marjan Ghazvininejad and Abdelrahman Mohamed and Omer Levy and Veselin Stoyanov and Luke Zettlemoyer},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages        = {7871--7880},
  year={2019}
}
@article{raffel2020exploringt5,
  title={Exploring the Limits of Transfer Learning with a Unified Text-to-text Transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={The Journal of Machine Learning Research},
  volume={21},
  number={1},
  pages={5485--5551},
  year={2020},
  publisher={JMLRORG}
}
@inproceedings{ma2021bprop,
  title={B-PROP: Bootstrapped Pre-training with Representative Words Prediction for Ad-hoc Retrieval},
  author={Ma, Xinyu and Guo, Jiafeng and Zhang, Ruqing and Fan, Yixing and Li, Yingyan and Cheng, Xueqi},
  booktitle={Proceedings of the 2021 ACM SIGIR International Conference on Theory of Information Retrieval},
  pages={1513--1522},
  year={2021}
}
@article{lin-2021-pretrained,
author = {Lin, Jimmy and Nogueira, Rodrigo and Yates, Andrew},
journal = {Synthesis Lectures on Human Language Technologies},
number = {4},
pages = {1--325},
publisher = {Morgan \& Claypool Publishers},
title = {Pretrained Transformers for Text Ranking: {BERT} and Beyond},
volume = {14},
year = {2021}}

@Misc{doct5querygit,
    author={Nogueira, Rodrigo and Lin, Jimmy},
    title = {DocT5query},
	howpublished = {\url{https://github.com/castorini/docTTTTTquery}},	
        year={2019}
}

@Misc{transformer-vae,
    key = {Transformer VAE},
    title = {A Library for Making Transformer Variational Autoencoders},
	howpublished = {\url{https://github.com/Fraser-Greenlee/transformer-vae}},	
    year={2020}
}

@Misc{doct5query-pseudo-queries-ms,
    title = {Pseudo queries for MSMARCO},
	howpublished = {\url{https://git.uwaterloo.ca/jimmylin/doc2query-data/raw/master/T5-doc/predicted_queries_doc.tar.gz}},	
        year={2019}
}

@Misc{t5base,
    author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
    title = {T5 Base},
	howpublished = {\url{https://huggingface.co/t5-base}},	
        year={2021}
}
@Misc{pytorch,
	howpublished = {\url{https://pytorch.org}},	
}
@Misc{transformers,
	howpublished = {\url{https://huggingface.co}},	
}

@inproceedings{chen-2023-unified,
    author = {Chen, Jiangui and Zhang, Ruqing and Guo, Jiafeng and de Rijke, Maarten and Liu, Yiqun and Fan, Yixing and Cheng, Xueqi},
    booktitle = {Proceedings of the 2023 ACM SIGIR International Conference on Theory of Information Retrieval},
    title = {A Unified Generative Retriever for Knowledge-Intensive Language Tasks via Prompt Learning},
    pages        = {1448--1457},
    year = {2023}
    }

@inproceedings{sun-2023-learning-arxiv,
    author = {Sun, Weiwei and Yan, Lingyong and Chen, Zheng and Wang, Shuaiqiang and Zhu, Haichao and Ren, Pengjie and Chen, Zhumin and Yin, Dawei and de Rijke, Maarten and Ren, Zhaochun},
    booktitle = {Thirty-seventh Conference on Neural Information Processing Systems},
    title = {Learning to Tokenize for Generative Retrieval},
    year = {2023}
    }


@inproceedings{hao2022teacher,
  title={Teacher Forcing Recovers Reward Functions for Text Generation},
  author={Hao, Yongchang and Liu, Yuxin and Mou, Lili},
  booktitle={Advances in neural information processing systems},
  year={2022}
}
@inproceedings{lin2022r,
  title={R-TeaFor: Regularized Teacher-Forcing for Abstractive Summarization},
  author={Lin, Guan-Yu and Cheng, Pu-Jen},
  booktitle={Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing},
  pages={6303--6311},
  year={2022}
}

@inproceedings{guu2020retrieval,
  title={Retrieval augmented language model pre-training},
  author={Guu, Kelvin and Lee, Kenton and Tung, Zora and Pasupat, Panupong and Chang, Mingwei},
  booktitle={International conference on machine learning},
  pages={3929--3938},
  year={2020},
  organization={PMLR}
}
@inproceedings{abnarexploring,
  title={Exploring the Limits of Large Scale Pre-training},
  author={Abnar, Samira and Dehghani, Mostafa and Neyshabur, Behnam and Sedghi, Hanie},
  booktitle={International Conference on Learning Representations},
  year={2022}
}
@inproceedings{lilarge,
  title={Large Language Models Can Be Strong Differentially Private Learners},
  author={Li, Xuechen and Tramer, Florian and Liang, Percy and Hashimoto, Tatsunori},
  booktitle={International Conference on Learning Representations},
  year={2022}

}
@inproceedings{weifinetuned,
  title={Finetuned Language Models are Zero-Shot Learners},
  author={Wei, Jason and Bosma, Maarten and Zhao, Vincent and Guu, Kelvin and Yu, Adams Wei and Lester, Brian and Du, Nan and Dai, Andrew M and Le, Quoc V},
  booktitle={International Conference on Learning Representations},
  year={2022}
}
@inproceedings{korbakreinforcement,
  title={On Reinforcement Learning and Distribution Matching for Fine-Tuning Language Models with no Catastrophic Forgetting},
  author={Korbak, Tomasz and Elsahar, Hady and Kruszewski, Germ{\'a}n and Dymetman, Marc},
  booktitle={Advances in neural information processing systems},
  year={2022}
}
@inproceedings{NEURIPS2021_0cd6a652,
 author = {Jaimovitch-Lopez, Gonzalo and Castellano Falc\'{o}n, David and Ferri, Cesar and Hern\'{a}ndez-Orallo, Jos\'{e}},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {1610--1623},
 publisher = {Curran Associates, Inc.},
 title = {Think Big, Teach Small: Do Language Models Distil Occam’s Razor?},
 year = {2021}
}
@inproceedings{NEURIPS2021_22b1f2e0,
 author = {Dong, Xinshuai and Luu, Anh Tuan and Lin, Min and Yan, Shuicheng and Zhang, Hanwang},
 booktitle = {Advances in Neural Information Processing Systems},
 title = {How Should Pre-Trained Language Models Be Fine-Tuned Towards Adversarial Robustness?},
 year = {2021}
}
@inproceedings{NEURIPS2021_86b3e165,
 author = {Wei, Colin and Xie, Sang Michael and Ma, Tengyu},
 booktitle = {Advances in neural information processing systems},
 title = {Why Do Pretrained Language Models Help in Downstream Tasks? An Analysis of Head and Prompt Tuning},
 volume = {34},
 year = {2021}
}
@inproceedings{balunovic2022lamp,
  title={Lamp: Extracting Text from Gradients with Language Model Priors},
  author={Balunovic, Mislav and Dimitrov, Dimitar and Jovanovi{\'c}, Nikola and Vechev, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022}
}
@inproceedings{khosla2020supervised,
  title={Supervised contrastive learning},
  author={Khosla, Prannay and Teterwak, Piotr and Wang, Chen and Sarna, Aaron and Tian, Yonglong and Isola, Phillip and Maschinot, Aaron and Liu, Ce and Krishnan, Dilip},
  booktitle={Advances in neural information processing systems},
  volume={33},
  pages={18661--18673},
  year={2020}
}
@inproceedings{tian2020makes,
  title={What makes for good views for contrastive learning?},
  author={Tian, Yonglong and Sun, Chen and Poole, Ben and Krishnan, Dilip and Schmid, Cordelia and Isola, Phillip},
  booktitle={Advances in neural information processing systems},
  volume={33},
  pages={6827--6839},
  year={2020}
}
@article{nadeem2022codedsi,
  title={{CodeDSI}: Differentiable Code Search},
  author={Nadeem, Usama and Ziems, Noah and Wu, Shaoen},
  journal={arXiv preprint arXiv:2210.00328},
  year={2022}
}
@article{rajput2023recommender,
  title={Recommender Systems with Generative Retrieval},
  author={Rajput, Shashank and Mehta, Nikhil and Singh, Anima and Keshavan, Raghunandan H and Vu, Trung and Heldt, Lukasz and Hong, Lichan and Tay, Yi and Tran, Vinh Q and Samost, Jonah and others},
  journal={arXiv preprint arXiv:2305.05065},
  year={2023}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
}

@inproceedings{pradeep2023does-scale-genir,
  title={How Does Generative Retrieval Scale to Millions of Passages?},
  author={Pradeep, Ronak and Hui, Kai and Gupta, Jai and Lelkes, Adam D. and Zhuang, Honglei and Lin, Jimmy and Metzler, Donald and Tran, Vinh Q.},
  booktitle={Gen-IR @ SIGIR 2023: The First Workshop on Generative Information Retrieval},
  year={2023}
}

@inproceedings{lang2022co,
  title={Co-training Improves Prompt-based Learning for Large Language Models},
  author={Lang, Hunter and Agrawal, Monica N and Kim, Yoon and Sontag, David},
  booktitle={International Conference on Machine Learning},
  year={2022},
}
@inproceedings{korbak2022controlling,
  title={Controlling Conditional Language Models without Catastrophic Forgetting},
  author={Korbak, Tomasz and Elsahar, Hady and Kruszewski, German and Dymetman, Marc},
  booktitle={International Conference on Machine Learning},
  pages={11499--11528},
  year={2022},
}
@inproceedings{lamprier2022generative,
  title={Generative Cooperative Networks for Natural Language Generation},
  author={Lamprier, Sylvain and Scialom, Thomas and Chaffin, Antoine and Claveau, Vincent and Kijak, Ewa and Staiano, Jacopo and Piwowarski, Benjamin},
  booktitle={International Conference on Machine Learning},
  pages={11891--11905},
  year={2022},

}
@inproceedings{lin2021generative,
  title={Generative Causal Explanations for Graph Neural Networks},
  author={Lin, Wanyu and Lan, Hao and Li, Baochun},
  booktitle={International Conference on Machine Learning},
  pages={6666--6679},
  year={2021},
  organization={PMLR}
}

@inproceedings{hudson2021generative,
  title={Generative Adversarial Transformers},
  author={Hudson, Drew A and Zitnick, Larry},
  booktitle={International conference on machine learning},
  pages={4487--4499},
  year={2021},
  organization={PMLR}
}
@inproceedings{zhang2021understanding,
  title={Understanding Failures in Out-of-Distribution Detection with Deep Generative Models},
  author={Zhang, Lily and Goldstein, Mark and Ranganath, Rajesh},
  booktitle={International conference on machine learning},
  year={2021},
  organization={PMLR}
}

@inproceedings{bae2022noisy,
  title={From Noisy Prediction to True Label: Noisy Prediction Calibration via Generative Model},
  author={Bae, HeeSun and Shin, Seungjae and Na, Byeonghu and Jang, JoonHo and Song, Kyungwoo and Moon, Il-Chul},
  booktitle={International Conference on Machine Learning},
  pages={1277--1297},
  year={2022},
  organization={PMLR}
}
@Misc{wikidump,
    author = {Wikipedia},
    title = {Data Dumps},
	howpublished = {\url{https://dumps.wikimedia.org/enwiki/latest/enwiki-latest-pages-articles.xml.bz2}},	
    year={2022}
}
@inproceedings{bendersky2010learning,
  title={Learning concept importance using a weighted dependence model},
  author={Bendersky, Michael and Metzler, Donald and Croft, W Bruce},
  booktitle={Proceedings of the third ACM international conference on Web search and data mining},
  pages={31--40},
  year={2010}
}
@inproceedings{bendersky2011parameterized,
  title={Parameterized concept weighting in verbose queries},
  author={Bendersky, Michael and Metzler, Donald and Croft, W Bruce},
  booktitle={Proceedings of the 34th international ACM SIGIR conference on Research and development in Information Retrieval},
  pages={605--614},
  year={2011}
}
@inproceedings{bendersky2012effective,
  title={Effective query formulation with multiple information sources},
  author={Bendersky, Michael and Metzler, Donald and Croft, W Bruce},
  booktitle={Proceedings of the fifth ACM international conference on Web search and data mining},
  pages={443--452},
  year={2012}
}
@inproceedings{lavrenko2017relevancequerylike,
  title={Relevance-based language models},
  author={Lavrenko, Victor and Croft, W Bruce},
  booktitle={ACM SIGIR Forum},
  volume={51},
  pages={260--267},
  year={2017},
  organization={ACM New York, NY, USA}
}
@inproceedings{lee2020contextualized,
  title={Contextualized Sparse Representations for Real-Time Open-Domain Question Answering},
  author={Lee, Jinhyuk and Seo, Minjoon and Hajishirzi, Hannaneh and Kang, Jaewoo},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={912--919},
  year={2020}
}
@inproceedings{tang2023semanticenhancedsedsi,
      title={Semantic-Enhanced Differentiable Search Index Inspired by Learning Strategies}, 
      author={Yubao Tang and Ruqing Zhang and Jiafeng Guo and Jiangui Chen and Zuowei Zhu and Shuaiqiang Wang and Dawei Yin and Xueqi Cheng},
      year={2023},
    booktitle={29th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
    pages={4904--4913},

}
@inproceedings{li2023multiview,
  title={Multiview Identifiers Enhanced Generative Retrieval},
  author={Li, Yongqi and Yang, Nan and Wang, Liang and Wei, Furu and Li, Wenjie},
  booktitle={61st Annual Meeting of the Association for Computational Linguistics},
  pages={6636--6648},
  year={2023}
}

@inproceedings{gao-etal-2019-jointly,
    title = "Jointly Optimizing Diversity and Relevance in Neural Response Generation",
    author = "Gao, Xiang  and
      Lee, Sungjin  and
      Zhang, Yizhe  and
      Brockett, Chris  and
      Galley, Michel  and
      Gao, Jianfeng  and
      Dolan, Bill",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/N19-1125",
    doi = "10.18653/v1/N19-1125",
    pages = "1229--1238",
}
@inproceedings{luan-etal-2017-multi,
    title = "Multi-Task Learning for Speaker-Role Adaptation in Neural Conversation Models",
    author = "Luan, Yi  and
      Brockett, Chris  and
      Dolan, Bill  and
      Gao, Jianfeng  and
      Galley, Michel",
    booktitle = "Proceedings of the Eighth International Joint Conference on Natural Language Processing",
    year = "2017",
    pages = "605--614",
}


@inproceedings{yamada2021efficient,
  title={Efficient Passage Retrieval with Hashing for Open-domain Question Answering},
  author={Yamada, Ikuya and Asai, Akari and Hajishirzi, Hannaneh},
  booktitle={Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing},
  pages={979--986},
  year={2021}
}
@inproceedings{zhou-2023-enhancing,
    author = {Zhou, Yujia and Dou, Zhicheng and Wen, Ji-Rong},
    title = {Enhancing Generative Retrieval with Reinforcement Learning from Relevance Feedback},
    booktitle = {EMNLP 2023: Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing},
    year = {2023},
}
@inproceedings{zhao2017learning,
  title={Learning Discourse-level Diversity for Neural Dialog Models using Conditional Variational Autoencoders},
  author={Zhao, Tiancheng and Zhao, Ran and Eskenazi, Maxine},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics},
  pages={654--664},
  year={2017}
}
@article{ji2020cross,
  title={Cross-modal guidance based auto-encoder for multi-video summarization},
  author={Ji, Zhong and Zhao, Yuxiao and Pang, Yanwei and Li, Xuelong},
  journal={Pattern Recognition Letters},
  volume={135},
  pages={131--137},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{wang2019topic,
  title={Topic-Guided Variational Autoencoders for Text Generation},
  author={Wang, Wenlin and Gan, Zhe and Xu, Hongteng and Zhang, Ruiyi and Wang, Guoyin and Shen, Dinghan and Chen, Changyou and Carin, Lawrence},
  booktitle={Proceedings of NAACL-HLT},
  pages={166--177},
  year={2019}
}

@inproceedings{zheng2021enhanced,
  title={Enhanced Seq2Seq Autoencoder via Contrastive Learning for Abstractive Text Summarization},
  author={Zheng, Chujie and Zhang, Kunpeng and Wang, Harry Jiannan and Fan, Ling and Wang, Zhe},
  booktitle={2021 IEEE International Conference on Big Data (Big Data)},
  pages={1764--1771},
  year={2021},
  organization={IEEE}
}
@inproceedings{liu2019transformer,
  title={A Transformer-based Variational Autoencoder for Sentence Generation},
  author={Liu, Danyang and Liu, Gongshen},
  booktitle={2019 International Joint Conference on Neural Networks},
  pages={1--7},
  year={2019},
  organization={IEEE}
}

@article{xu2019adversarially,
  title={Adversarially Approximated Autoencoder for Image Generation and Manipulation},
  author={Xu, Wenju and Keshmiri, Shawn and Wang, Guanghui},
  journal={IEEE Transactions on Multimedia},
  volume={21},
  number={9},
  pages={2387--2396},
  year={2019},
  publisher={IEEE}
}
@inproceedings{chu2021evaluating,
  title={Evaluating Relevance Judgments with Pairwise Discriminative Power},
  author={Chu, Zhumin and Mao, Jiaxin and Zhang, Fan and Liu, Yiqun and Sakai, Tetsuya and Zhang, Min and Ma, Shaoping},
  booktitle={Proceedings of the 30th ACM International Conference on Information \& Knowledge Management},
  pages={261--270},
  year={2021}
}
@inproceedings{lan2014position,
  title={Position-Aware ListMLE: A Sequential Learning Process for Ranking.},
  author={Lan, Yanyan and Zhu, Yadong and Guo, Jiafeng and Niu, Shuzi and Cheng, Xueqi},
  booktitle={UAI},
  volume={14},
  pages={449--458},
  year={2014}
}
@inproceedings{szummer2011semi,
  title={Semi-supervised learning to rank with preference regularization},
  author={Szummer, Martin and Yilmaz, Emine},
  booktitle={Proceedings of the 20th ACM international conference on Information and knowledge management},
  pages={269--278},
  year={2011}
}
@article{formal2021splade-v2,
  title={SPLADE v2: Sparse Lexical and Expansion Model for Information Retrieval},
  author={Formal, Thibault and Lassance, Carlos and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  journal={arXiv preprint arXiv:2109.10086},
  year={2021}
}
@inproceedings{formal2021splade,
  title={SPLADE: Sparse Lexical and Expansion Model for First Stage Ranking},
  author={Formal, Thibault and Piwowarski, Benjamin and Clinchant, St{\'e}phane},
  booktitle={Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={2288--2292},
  year={2021}
}

@inproceedings{wang2023novo,
  title={NOVO: Learnable and Interpretable Document Identifiers for Model-Based {IR}},
  author={Wang, Zihan and Zhou, Yujia and Tu, Yiteng and Dou, Zhicheng},
  booktitle={32nd ACM International Conference on Information and Knowledge Management  },
  pages = {2656--2665},
  year={2023}
}
@inproceedings{naseri2021ceqe,
  title={Ceqe: Contextualized Embeddings for Query Expansion},
  author={Naseri, Shahrzad and Dalton, Jeffrey and Yates, Andrew and Allan, James},
  booktitle={Advances in Information Retrieval: 43rd European Conference on IR Research},
  pages={467--482},
  year={2021},
  organization={Springer}
}
@inproceedings{huston2014comparison,
  title={A Comparison of Retrieval Models Using Term Dependencies},
  author={Huston, Samuel and Croft, W Bruce},
  booktitle={Proceedings of the 23rd ACM International Conference on Conference on Information and Knowledge Management},
  pages={111--120},
  year={2014}
}
@inproceedings{nguyen2023generative-genir,
  title={Generative Retrieval as Dense Retrieval},
  author={Nguyen, Thong and Yates, Andrew},
  booktitle={Gen-IR @ SIGIR 2023: The First Workshop on Generative Information Retrieval},
  year={2023}
}
@inproceedings{li2024learning,
  title={Learning to rank in generative retrieval},
  author={Li, Yongqi and Yang, Nan and Wang, Liang and Wei, Furu and Li, Wenjie},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={8716--8723},
  year={2024}
}
@inproceedings{yang2023auto,
  title={Auto Search Indexer for End-to-End Document Retrieval},
  author={Yang, Tianchi and Song, Minghui and Zhang, Zihan and Huang, Haizhen and Deng, Weiwei and Sun, Feng and Zhang, Qi},
  booktitle={Findings of the Association for Computational Linguistics: EMNLP 2023},
  year={2023}
}
@article{tang2024listwise,
  title={Listwise Generative Retrieval Models via a Sequential Learning Process},
  author={Tang, Yubao and Zhang, Ruqing and Guo, Jiafeng and de Rijke, Maarten and Chen, Wei and Cheng, Xueqi},
  journal={ACM Transactions on Information Systems},
  year={2024},
  publisher={ACM New York, NY}
}
@inproceedings{tang2023recent,
  title={Recent Advances in Generative Information Retrieval},
  author={Tang, Yubao and Zhang, Ruqing and Guo, Jiafeng and de Rijke, Maarten},
  booktitle={Proceedings of the Annual International ACM SIGIR Conference on Research and Development in Information Retrieval in the Asia Pacific Region},
  pages={294--297},
  year={2023}
}
@inproceedings{ren2023tome,
  title={TOME: a Two-stage Approach for Model-based Retrieval},
  author={Ren, Ruiyang and Zhao, Wayne Xin and Liu, Jing and Wu, Hua and Wen, Ji-Rong and Wang, Haifeng},
   booktitle    = {Proceedings of the 61st Annual Meeting of the Association for Computational Linguistics},
  pages        = {6102--6114},
  year={2023},
}

@article{zhang2023term-sets-arxiv,
  title={Term-Sets Can Be Strong Document Identifiers For Auto-Regressive Search Engines},
  author={Zhang, Peitian and Liu, Zheng and Zhou, Yujia and Dou, Zhicheng and Cao, Zhao},
  journal={arXiv preprint arXiv:2305.13859},
  year={2023}
}
@inproceedings{zhang2024term,
  title={Generative Retrieval via Term Set Generation},
  author={Zhang, Peitian and Liu, Zheng and Zhou, Yujia and Dou, Zhicheng and Cao, Zhao},
  booktitle={Proceedings of the 2024 ACM SIGIR International Conference on Theory of Information Retrieva},
  year={2024}
}

@inproceedings{zeng2024planning,
  title={Planning Ahead in Generative Retrieval: Guiding Autoregressive Generation through Simultaneous Decoding},
  author={Zeng, Hansi and Luo, Chen and Zamani, Hamed},
  booktitle={Proceedings of the 2024 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2024}
}

@inproceedings{zhou2023enhancing,
  title={Enhancing Generative Retrieval with Reinforcement Learning from Relevance Feedback},
  author={Zhou, Yujia and Dou, Zhicheng and Wen, Ji-Rong},
  booktitle={Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing},
  pages={12481--12490},
  year={2023}
}
@inproceedings{zeng2023scalable,
  title={Scalable and Effective Generative Information Retrieval},
  author={Zeng, Hansi and Luo, Chen and Jin, Bowen and Sarwar, Sheikh Muhammad and Wei, Tianxin and Zamani, Hamed},
  booktitle={The Web Conference},
  year={2024}
}
@inproceedings{chen2023-continual,
  title={Continual Learning for Generative Retrieval over Dynamic Corpora},
  author={Chen, Jiangui and Zhang, Ruqing and Guo, Jiafeng and de Rijke, Maarten and Chen, Wei and Fan, Yixing and Cheng, Xueqi},
  booktitle    = {Proceedings of the 32nd {ACM} International Conference on Information and Knowledge Management},
  pages = {306–315},
  year={2023}
}
@article{pan2002maximum,
  title={Maximum Likelihood Estimation},
  author={Pan, Jian-Xin and Fang, Kai-Tai and Pan, Jian-Xin and Fang, Kai-Tai},
  journal={Growth curve models and statistical diagnostics},
  pages={77--158},
  year={2002},
  publisher={Springer}
}

